Simple, Efficient, and Neural Algorithms for Sparse Coding

Sparse coding is a basic task in many fields including signal processing, neuroscience and machine learning where the goal is to learn a basis that enables a sparse representation of a given set of data, if one exists. Its standard formulation is as a non-convex optimization problem which is solved in practice by heuristics based on alternating minimization. Re- cent work has resulted in several algorithms for sparse coding with provable guarantees, but somewhat surprisingly these are outperformed by the simple alternating minimization heuristics. Here we give a general framework for understanding alternating minimization which we leverage to analyze existing heuristics and to design new ones also with provable guarantees. Some of these algorithms seem implementable on simple neural architectures, which was the original motivation of Olshausen and Field (1997a) in introducing sparse coding. We also give the first efficient algorithm for sparse coding that works almost up to the information theoretic limit for sparse recovery on incoherent dictionaries. All previous algorithms that approached or surpassed this limit run in time exponential in some natural parameter. Finally, our algorithms improve upon the sample complexity of existing approaches. We believe that our analysis framework will have applications in other settings where simple iterative algorithms are used.

==> convexityflat.tex <==

\subsection{Approximate Gradient Descent; proof of Theorem~\ref{thm:tiger-convergence}} \label{sec:framework}

\iffalse 
Many variants of gradient descent are known to quickly converge to the global minimum when applied to a strongly convex function $f(z)$. 
Stochastic gradient descent is widely popular in machine learning because it only needs an estimate whose {\em expectation} is the true gradient. In our setting, even the expectation of our estimate will be biased, but we give general conditions --- reminiscent of Lyapunov functions used in study of dynamical systems --- that implies convergence to a particular
desired solution  $z^*$. At step $s$ the algorithm starts with $z^s$, computes some direction $g^s$, and updates its estimate in the following manner: $z^{s+1} = z^s - \eta g^s$.


\begin{definition}[{\bf Condition 1}]\label{eqn:con}
A vector $g^s$ {\em $(\alpha, \beta,\epsilon_s)$-correlated with} $z^*$ if
$$ \langle g^s, z^s-z^*\rangle \ge \alpha \|z^s-z^*\|^2 + \beta\|g^s\|^2 - \epsilon_s.$$
\end{definition}
\noindent{\em Remark:} The traditional analysis of convex optimization corresponds to the setting where $z^*$ is the global optimal of some convex function $f$, and $\epsilon_s = 0$. Specifically, if $f(\cdot)$ is $2\alpha$-convex and $1/(2\beta)$-smooth, then $g^s = \nabla f(z^s)$ $(\alpha,\beta,0)$-correlated with $z^*$. 

% Under the above condition, we have the following theorem:
% In the previous section we gave update rules derived from $\nabla \widetilde{f}(B)$ that satisfy Condition~\ref{eqn:con}, and here we give a general analysis of their convergence. Our main theorem is:


\begin{theorem}\label{thm:tiger-convergence}
Suppose $g^s$ satisfies Definition~\ref{eqn:con} for $s = 1,2,\dots,T$, and $\eta$ satisfies  $0< \eta \le 2\beta$ and $\epsilon =  \max_{s=1}^{T} \epsilon_s$. 
Then for any $s = 1,\dots,T$, 
$$ \| z^{s+1}-z^*\|^2 \leq (1-2\alpha\eta) \|z^s-z^*\|^2 + 2\eta \epsilon_s$$
In particular, the update rule above converges to $z^*$ geometrically with systematic error $\epsilon/\alpha$ in the sense that 
%$$\|z_s-z^*\|^2 \le (1-2\alpha\eta)^s \|z_0-z^*\| + \epsilon/\alpha.$$
$$\|z^s-z^*\|^2 \le (1-2\alpha\eta)^s \|z^0-z^*\|^2 + \epsilon/\alpha.$$
Furthermore, if $\epsilon_s < \frac{\alpha}{2} \|z^s-z^*\|^2$ for $s = 1,\dots,T$, then 
$$\|z^s-z^*\|^2 \le (1-\alpha\eta)^s \|z^0-z^*\|^2.$$
%$$\|x^s-x^*\|^2 \le (1-2\alpha\beta)^s R^2$$
\end{theorem}
\fi 

\begin{proof}[Proof of Theorem~\ref{thm:tiger-convergence}]
We expand the error as
\[
\begin{array}{rl}
\|z^{s+1} - z^*\|^2  &=  \|z^s-z^*\|^2 -2 \eta {g^s}^T(z^s-z^*) + \eta^2 \|g^s\|^2\\
 &= \|z^s-z^*\|^2 -\eta \left(2{g^s}^T(z^s-z^*) -\eta \|g^s\|^2\right) \\
&\leq \|z^s-z^*\|^2 -\eta \left(2\alpha \|z^s-z^*\|^2 + (2\beta -\eta)\|g^s\|^2-2\epsilon_s\right) \quad \mbox{(Definition~\ref{eqn:con} and  $\eta \le 2 \beta$)}  \\
&\leq \|z^s-z^*\|^2 -\eta \left(2\alpha \|z^s-z^*\|^2 -2\epsilon_s\right) \\
& \leq (1-2\alpha\eta) \|z^s-z^*\|^2 + 2\eta \epsilon_s
\end{array}
\]
%\Tnote{The proof might need slight change if we agree with the new phrasing of the statement.}
Then solving this recurrence we have
$\|z^{s+1}-z^*\|^2  \leq (1-2\alpha\eta)^{s+1} R^2 + \frac{\epsilon}{\alpha}$
where $R = \|z^0-z^* \|$. And furthermore if $\epsilon_s < \frac{\alpha}{2} \|z^s-z^*\|^2$ we have instead
$$ \|z^{s+1} - z^*\|^2 \leq (1-2\alpha\eta) \|z^s-z\|^2 + \alpha \eta \|z^s-z\|^2 = (1-\alpha\eta) \|z^s-z\|^2$$
and this yields the second part of the theorem too.
\end{proof}

In fact, we can extend the analysis above to obtain identical results for the case of constrained optimization. Suppose we are interested in optimizing a convex function $f(z)$ over a convex set $\mathcal{B}$. 
The standard approach is to take a step in the direction of the gradient (or $g^s$ in our case) and then project into $\mathcal{B}$ after each iteration,
namely, replace $z^{s+1}$ by $\mbox{Proj}_\mathcal{B}\, z^{s+1}$ which is the closest point in $\mathcal{B}$ to $z^{s+1}$ in Euclidean distance.
 It is well-known that if $z^*\in \mathcal{B}$, then $\|\mbox{Proj}_\mathcal{B}\; z - z^*\| \le \|z - z^*\|$. Therefore we obtain the following as an immediate corollary to the above analysis:

\begin{corollary}\label{cor:tiger-convexity}
Suppose $g^s$ satisfies Definition~\ref{eqn:con} for $s = 1,2, \dots,T$ and set  $0< \eta \le 2\beta$ and $\epsilon =  \max_{s=1}^T \epsilon_s$. Further suppose that
$z^*$ lies in a  convex set $\mathcal{B}$. Then the update rule $z^{s+1} = \mbox{Proj}_\mathcal{B}(z^s - \eta g^s)$ satisfies that for any $s = 1,\dots,T$, 
$$\|z^s-z^*\|^2 \le (1-2\alpha\eta)^s \|z^0-z^*\| + \epsilon/\alpha$$
In particular, $z^s$ converges to $z^*$ geometrically with systematic error $\epsilon/\alpha$. 
%$$\|x^s-x^*\|^2 \le (1-4\alpha\beta)^s \|z^0-z^*\| + \epsilon/(\alpha)$$
Additionally if $\epsilon_s < \frac{\alpha}{2} \|z^s-z^*\|^2$ for $s = 1,\dots,T$, then 
$$\|z^s-z^*\|^2 \le (1-\alpha\eta)^s \|z^0-z^*\|^2$$
%$$\|x^s-x^*\|^2 \le (1-2\alpha\beta)^s R^2$$
\end{corollary}

What remains is to derive a functional form for various update rules and show that these rules move in a direction $g^s$ that approximately points in the direction of the desired solution $z^*$ (under the assumption that our data is generated from a stochastic model that meets certain conditions). 

%The main reason we need the use the framework above is that in our applications we have
%$$f(B) = \E[\|y-Bx\|^2]$$
%which is a convex function, but the catch is that for each example $y$ we do not know its representation $x$. Hence we cannot compute $\nabla f(B)$. Our hope is that if we get an estimate $\widetilde{x}$ for $x$ we can plug in $\widetilde{x}$ for $x$ to get
%$$\widetilde{f}(B) = \E[\|y-B\widetilde{x}\|^2]$$
%and take its gradient instead.




%However, recall in our applications we have
%$f(B) = \E[\|y-Bx\|^2]$ which is a convex function, but we don't know how to compute its true gradient. Later we will introduce different %rules that have different $\epsilon$'s, and show that $\epsilon$'s are small enough to guarantee convergence.

%\noindent The proof of this theorem is standard; it is our abstraction of when it works that is new. In particular if $f(z)$ is $2\alpha$-convex and $1/(2\beta)$-smooth, then $g_s = \nabla f(z_s)$ satisfies Condition~\ref{eqn:con} with $\epsilon_s = 0$ and we recover various well-known results as a special case. Additionally, we can use the standard analysis for the non-smooth case to extract similar conditions with slower convergence rates too. But the above will be sufficient for our purposes. 

%One could see that if $f$ is $2\alpha$-convex and $1/(2\beta)$-smooth, then $g_s = \nabla f(x_s)$ satisfies Condition~\ref{eqn:con} with $\epsilon_s = 0$. Also if there is a constrained set $\mathcal{X}$, then the gradient proxy $g_{\mathcal{X}}$ also satisfies Condition~\ref{eqn:con} with $\epsilon_s = 0$. (Gradient proxy is roughly defined as the difference between $x_{s+1}$ and $x_s$ using projected gradient descent. ) Therefore, this captures the typical convexity and exact gradient case. For non-smooth cases we actually could also extract similar conditions with slower convergence guarantees. But in this writeup we only deal with the case when geometrical decay of error is possible. 

%We remark that Condition~\ref{eqn:con} also works well with projection. In particular, if we are interested in constrained optimization over a set $\mathcal{Z}$, and the update rule is instead
%$$z_{s+1} = \Pi_{\mathcal{Z}}(z_s -\eta g_s)$$
%%$$x_{s+1} = Proj_{\mathcal{X}}(x_s -2\beta g_s)$$
%we can define a gradient proxy as $g_{\mathcal{Z},s} = (z_{s+1}-z_s)/\eta$. And if $g_s$ satisfies Condition~\ref{eqn:con}, so does $g_{\mathcal{Z},s}$. 

\iffalse 
\begin{proof}
We expand the error as
\[
\begin{array}{rl}
\|z_{s+1} - z^*\|^2  &=  \|z_s-z^*\|^2 -2 \eta g_s^T(z_s-z^*) + \eta^2 \|g_s\|^2\\
 &= \|z_s-z^*\|^2 -\eta \left(2g_s^T(z_s-z^*) -\eta \|g_s\|^2\right) \\
&\leq \|z_s-z^*\|^2 -\eta \left(2\alpha \|z_s-z^*\|^2 + (2\beta -\eta)\|g_s\|^2-2\epsilon_s\right) \quad \mbox{(Definition~\ref{eqn:con} and  $\eta \le 2 \beta$)}  \\
&\leq \|z_s-z^*\|^2 -\eta \left(2\alpha \|z_s-z^*\|^2 -2\epsilon_s\right) \\
& \leq (1-2\alpha\eta) \|z_s-z^*\|^2 + 2\eta \epsilon_s
\end{array}
\]
\Tnote{The proof might need slight change if we agree with the new phrasing of the statement.}
Then solving this recurrence we have
$\|z_{s+1}-z^*\|^2  \leq (1-2\alpha\eta)^{s+1} R^2 + \frac{\epsilon}{\alpha}$
where $R = \|z_0-z^* \|$. And furthermore if $\epsilon_s < \frac{\alpha}{2} \|z_s-z^*\|^2$ we have instead
$$ \|z_{s+1} - z^*\|^2 \leq (1-2\alpha\eta) \|z_s-z\|^2 + \alpha \eta \|z_s-z\|^2 = (1-\alpha\eta) \|z_s-z\|^2$$
and this yields the second part of the theorem too.
\end{proof}

In fact, we can extend the analysis above to obtain identical results for the case of constrained optimization. Suppose we are interested in optimizing a convex function $f(z)$ over a convex set $\mathcal{B}$. 
The standard approach is to take a step in the direction of the gradient (or $g_s$ in our case) and then project into $\mathcal{B}$ after each iteration,
namely, replace $z_{s+1}$ by $\mbox{Proj}_\mathcal{B}\, z_{s+1}$ which is the closest point in $\mathcal{B}$ to $z_{s+1}$ in Euclidean distance.
 It is well-known that if $z^*\in \mathcal{B}$, then $\|\mbox{Proj}_\mathcal{B}\; z - z^*\| \le \|z - z^*\|$. Therefore we obtain the following as an immediate corollary to the above analysis:

\begin{corollary}
Suppose $g_s$ satisfies Definition~\ref{eqn:con} for $s = 1,2, \dots,T$ and set  $0< \eta \le 2\beta$ and $\epsilon =  \max_{s=1}^T \epsilon_s$. Further suppose that
$z^*$ lies in a  convex set $\mathcal{B}$. Then the update rule $z_{s+1} = \mbox{Proj}_\mathcal{B}(z_s - \eta g_s)$ satisfies that for any $s = 1,\dots,T$, 
$$\|z_s-z^*\|^2 \le (1-2\alpha\eta)^s \|z_0-z^*\| + \epsilon/\alpha$$
In particular, $z^s$ converges to $z^*$ geometrically with systematic error $\epsilon/\alpha$. 
%$$\|x_s-x^*\|^2 \le (1-4\alpha\beta)^s \|z_0-z^*\| + \epsilon/(\alpha)$$
Additionally if $\epsilon_s < \frac{\alpha}{2} \|z_s-z^*\|^2$ for $s = 1,\dots,T$, then 
$$\|z_s-z^*\|^2 \le (1-\alpha\eta)^s \|z_0-z^*\|$$
%$$\|x_s-x^*\|^2 \le (1-2\alpha\beta)^s R^2$$
\end{corollary}

\fi 

==> convexityflat10.tex <==

\section{Approximate Gradient Descent} \label{sec:framework}

Here we prove Theorem~\ref{thm:tiger-convergence}:

\iffalse 
Many variants of gradient descent are known to quickly converge to the global minimum when applied to a strongly convex function $f(z)$. 
Stochastic gradient descent is widely popular in machine learning because it only needs an estimate whose {\em expectation} is the true gradient. In our setting, even the expectation of our estimate will be biased, but we give general conditions --- reminiscent of Lyapunov functions used in study of dynamical systems --- that implies convergence to a particular
desired solution  $z^*$. At step $s$ the algorithm starts with $z^s$, computes some direction $g^s$, and updates its estimate in the following manner: $z^{s+1} = z^s - \eta g^s$.


\begin{definition}[{\bf Condition 1}]\label{eqn:con}
A vector $g^s$ {\em $(\alpha, \beta,\epsilon_s)$-correlated with} $z^*$ if
$$ \langle g^s, z^s-z^*\rangle \ge \alpha \|z^s-z^*\|^2 + \beta\|g^s\|^2 - \epsilon_s.$$
\end{definition}
\noindent{\em Remark:} The traditional analysis of convex optimization corresponds to the setting where $z^*$ is the global optimal of some convex function $f$, and $\epsilon_s = 0$. Specifically, if $f(\cdot)$ is $2\alpha$-convex and $1/(2\beta)$-smooth, then $g^s = \nabla f(z^s)$ $(\alpha,\beta,0)$-correlated with $z^*$. 

% Under the above condition, we have the following theorem:
% In the previous section we gave update rules derived from $\nabla \widetilde{f}(B)$ that satisfy Condition~\ref{eqn:con}, and here we give a general analysis of their convergence. Our main theorem is:


\begin{theorem}\label{thm:tiger-convergence}
Suppose $g^s$ satisfies Definition~\ref{eqn:con} for $s = 1,2,\dots,T$, and $\eta$ satisfies  $0< \eta \le 2\beta$ and $\epsilon =  \max_{s=1}^{T} \epsilon_s$. 
Then for any $s = 1,\dots,T$, 
$$ \| z^{s+1}-z^*\|^2 \leq (1-2\alpha\eta) \|z^s-z^*\|^2 + 2\eta \epsilon_s$$
In particular, the update rule above converges to $z^*$ geometrically with systematic error $\epsilon/\alpha$ in the sense that 
%$$\|z_s-z^*\|^2 \le (1-2\alpha\eta)^s \|z_0-z^*\| + \epsilon/\alpha.$$
$$\|z^s-z^*\|^2 \le (1-2\alpha\eta)^s \|z^0-z^*\|^2 + \epsilon/\alpha.$$
Furthermore, if $\epsilon_s < \frac{\alpha}{2} \|z^s-z^*\|^2$ for $s = 1,\dots,T$, then 
$$\|z^s-z^*\|^2 \le (1-\alpha\eta)^s \|z^0-z^*\|^2.$$
%$$\|x^s-x^*\|^2 \le (1-2\alpha\beta)^s R^2$$
\end{theorem}
\fi 

\begin{proof}[Proof of Theorem~\ref{thm:tiger-convergence}]
We expand the error as
\[
\begin{array}{rl}
\|z^{s+1} - z^*\|^2  &=  \|z^s-z^*\|^2 -2 \eta {g^s}^T(z^s-z^*) + \eta^2 \|g^s\|^2\\
 &= \|z^s-z^*\|^2 -\eta \left(2{g^s}^T(z^s-z^*) -\eta \|g^s\|^2\right) \\
&\leq \|z^s-z^*\|^2 -\eta \left(2\alpha \|z^s-z^*\|^2 + (2\beta -\eta)\|g^s\|^2-2\epsilon_s\right) \quad \mbox{(Definition~\ref{eqn:con} and  $\eta \le 2 \beta$)}  \\
&\leq \|z^s-z^*\|^2 -\eta \left(2\alpha \|z^s-z^*\|^2 -2\epsilon_s\right) \\
& \leq (1-2\alpha\eta) \|z^s-z^*\|^2 + 2\eta \epsilon_s
\end{array}
\]
%\Tnote{The proof might need slight change if we agree with the new phrasing of the statement.}
Then solving this recurrence we have
$\|z^{s+1}-z^*\|^2  \leq (1-2\alpha\eta)^{s+1} R^2 + \frac{\epsilon}{\alpha}$
where $R = \|z^0-z^* \|$. And furthermore if $\epsilon_s < \frac{\alpha}{2} \|z^s-z^*\|^2$ we have instead
$$ \|z^{s+1} - z^*\|^2 \leq (1-2\alpha\eta) \|z^s-z\|^2 + \alpha \eta \|z^s-z\|^2 = (1-\alpha\eta) \|z^s-z\|^2$$
and this yields the second part of the theorem too.
\end{proof}

In fact, we can extend the analysis above to obtain identical results for the case of constrained optimization. Suppose we are interested in optimizing a convex function $f(z)$ over a convex set $\mathcal{B}$. 
The standard approach is to take a step in the direction of the gradient (or $g^s$ in our case) and then project into $\mathcal{B}$ after each iteration,
namely, replace $z^{s+1}$ by $\mbox{Proj}_\mathcal{B}\, z^{s+1}$ which is the closest point in $\mathcal{B}$ to $z^{s+1}$ in Euclidean distance.
 It is well-known that if $z^*\in \mathcal{B}$, then $\|\mbox{Proj}_\mathcal{B}\; z - z^*\| \le \|z - z^*\|$. Therefore we obtain the following as an immediate corollary to the above analysis:

\begin{corollary}\label{cor:tiger-convexity}
Suppose $g^s$ satisfies Definition~\ref{eqn:con} for $s = 1,2, \dots,T$ and set  $0< \eta \le 2\beta$ and $\epsilon =  \max_{s=1}^T \epsilon_s$. Further suppose that
$z^*$ lies in a  convex set $\mathcal{B}$. Then the update rule $z^{s+1} = \mbox{Proj}_\mathcal{B}(z^s - \eta g^s)$ satisfies that for any $s = 1,\dots,T$, 
$$\|z^s-z^*\|^2 \le (1-2\alpha\eta)^s \|z^0-z^*\|^2 + \epsilon/\alpha$$
In particular, $z^s$ converges to $z^*$ geometrically with systematic error $\epsilon/\alpha$. 
%$$\|x^s-x^*\|^2 \le (1-4\alpha\beta)^s \|z^0-z^*\| + \epsilon/(\alpha)$$
Additionally if $\epsilon_s < \frac{\alpha}{2} \|z^s-z^*\|^2$ for $s = 1,\dots,T$, then 
$$\|z^s-z^*\|^2 \le (1-\alpha\eta)^s \|z^0-z^*\|^2$$
%$$\|x^s-x^*\|^2 \le (1-2\alpha\beta)^s R^2$$
\end{corollary}

What remains is to derive a functional form for various update rules and show that these rules move in a direction $g^s$ that approximately points in the direction of the desired solution $z^*$ (under the assumption that our data is generated from a stochastic model that meets certain conditions). 

%The main reason we need the use the framework above is that in our applications we have
%$$f(B) = \E[\|y-Bx\|^2]$$
%which is a convex function, but the catch is that for each example $y$ we do not know its representation $x$. Hence we cannot compute $\nabla f(B)$. Our hope is that if we get an estimate $\widetilde{x}$ for $x$ we can plug in $\widetilde{x}$ for $x$ to get
%$$\widetilde{f}(B) = \E[\|y-B\widetilde{x}\|^2]$$
%and take its gradient instead.




%However, recall in our applications we have
%$f(B) = \E[\|y-Bx\|^2]$ which is a convex function, but we don't know how to compute its true gradient. Later we will introduce different %rules that have different $\epsilon$'s, and show that $\epsilon$'s are small enough to guarantee convergence.

%\noindent The proof of this theorem is standard; it is our abstraction of when it works that is new. In particular if $f(z)$ is $2\alpha$-convex and $1/(2\beta)$-smooth, then $g_s = \nabla f(z_s)$ satisfies Condition~\ref{eqn:con} with $\epsilon_s = 0$ and we recover various well-known results as a special case. Additionally, we can use the standard analysis for the non-smooth case to extract similar conditions with slower convergence rates too. But the above will be sufficient for our purposes. 

%One could see that if $f$ is $2\alpha$-convex and $1/(2\beta)$-smooth, then $g_s = \nabla f(x_s)$ satisfies Condition~\ref{eqn:con} with $\epsilon_s = 0$. Also if there is a constrained set $\mathcal{X}$, then the gradient proxy $g_{\mathcal{X}}$ also satisfies Condition~\ref{eqn:con} with $\epsilon_s = 0$. (Gradient proxy is roughly defined as the difference between $x_{s+1}$ and $x_s$ using projected gradient descent. ) Therefore, this captures the typical convexity and exact gradient case. For non-smooth cases we actually could also extract similar conditions with slower convergence guarantees. But in this writeup we only deal with the case when geometrical decay of error is possible. 

%We remark that Condition~\ref{eqn:con} also works well with projection. In particular, if we are interested in constrained optimization over a set $\mathcal{Z}$, and the update rule is instead
%$$z_{s+1} = \Pi_{\mathcal{Z}}(z_s -\eta g_s)$$
%%$$x_{s+1} = Proj_{\mathcal{X}}(x_s -2\beta g_s)$$
%we can define a gradient proxy as $g_{\mathcal{Z},s} = (z_{s+1}-z_s)/\eta$. And if $g_s$ satisfies Condition~\ref{eqn:con}, so does $g_{\mathcal{Z},s}$. 

\iffalse 
\begin{proof}
We expand the error as
\[
\begin{array}{rl}
\|z_{s+1} - z^*\|^2  &=  \|z_s-z^*\|^2 -2 \eta g_s^T(z_s-z^*) + \eta^2 \|g_s\|^2\\
 &= \|z_s-z^*\|^2 -\eta \left(2g_s^T(z_s-z^*) -\eta \|g_s\|^2\right) \\
&\leq \|z_s-z^*\|^2 -\eta \left(2\alpha \|z_s-z^*\|^2 + (2\beta -\eta)\|g_s\|^2-2\epsilon_s\right) \quad \mbox{(Definition~\ref{eqn:con} and  $\eta \le 2 \beta$)}  \\
&\leq \|z_s-z^*\|^2 -\eta \left(2\alpha \|z_s-z^*\|^2 -2\epsilon_s\right) \\
& \leq (1-2\alpha\eta) \|z_s-z^*\|^2 + 2\eta \epsilon_s
\end{array}
\]
\Tnote{The proof might need slight change if we agree with the new phrasing of the statement.}
Then solving this recurrence we have
$\|z_{s+1}-z^*\|^2  \leq (1-2\alpha\eta)^{s+1} R^2 + \frac{\epsilon}{\alpha}$
where $R = \|z_0-z^* \|$. And furthermore if $\epsilon_s < \frac{\alpha}{2} \|z_s-z^*\|^2$ we have instead
$$ \|z_{s+1} - z^*\|^2 \leq (1-2\alpha\eta) \|z_s-z\|^2 + \alpha \eta \|z_s-z\|^2 = (1-\alpha\eta) \|z_s-z\|^2$$
and this yields the second part of the theorem too.
\end{proof}

In fact, we can extend the analysis above to obtain identical results for the case of constrained optimization. Suppose we are interested in optimizing a convex function $f(z)$ over a convex set $\mathcal{B}$. 
The standard approach is to take a step in the direction of the gradient (or $g_s$ in our case) and then project into $\mathcal{B}$ after each iteration,
namely, replace $z_{s+1}$ by $\mbox{Proj}_\mathcal{B}\, z_{s+1}$ which is the closest point in $\mathcal{B}$ to $z_{s+1}$ in Euclidean distance.
 It is well-known that if $z^*\in \mathcal{B}$, then $\|\mbox{Proj}_\mathcal{B}\; z - z^*\| \le \|z - z^*\|$. Therefore we obtain the following as an immediate corollary to the above analysis:

\begin{corollary}
Suppose $g_s$ satisfies Definition~\ref{eqn:con} for $s = 1,2, \dots,T$ and set  $0< \eta \le 2\beta$ and $\epsilon =  \max_{s=1}^T \epsilon_s$. Further suppose that
$z^*$ lies in a  convex set $\mathcal{B}$. Then the update rule $z_{s+1} = \mbox{Proj}_\mathcal{B}(z_s - \eta g_s)$ satisfies that for any $s = 1,\dots,T$, 
$$\|z_s-z^*\|^2 \le (1-2\alpha\eta)^s \|z_0-z^*\| + \epsilon/\alpha$$
In particular, $z^s$ converges to $z^*$ geometrically with systematic error $\epsilon/\alpha$. 
%$$\|x_s-x^*\|^2 \le (1-4\alpha\beta)^s \|z_0-z^*\| + \epsilon/(\alpha)$$
Additionally if $\epsilon_s < \frac{\alpha}{2} \|z_s-z^*\|^2$ for $s = 1,\dots,T$, then 
$$\|z_s-z^*\|^2 \le (1-\alpha\eta)^s \|z_0-z^*\|$$
%$$\|x_s-x^*\|^2 \le (1-2\alpha\beta)^s R^2$$
\end{corollary}

\fi 

==> indicatorincludeflat.tex <==
\section{A Neurally Plausible Algorithm with Provable Guarantees}\label{sec:update_rule}
Here we will design and analyze a neurally plausible algorithm for sparse coding.  The algorithm is given in Algorithm~\ref{eqn:simplestupdate}. Moreover it makes use of just matrix multiplication and thresholding. These are both operations that neurons can implement, and we go further and give an architecture implementing our algorithm as was done in \cite{OF}.  The fact that such a simple algorithm works sheds new light on how sparse coding might be accomplished in nature. 

Here and throughout this paper we will work with the following measure of closeness:

\begin{definition}\label{def:near}
$\tilA$ is $(\delta, \kappa)$-\near to $\trA$ if there is a permutation $\pi: [m] \rightarrow [m]$ and a choice of signs $\sigma: [m] \rightarrow \{\pm 1\}$ such that
$$ \|\sigma(i) \tilA_{\pi(i)} - \trA_i\| \leq \delta \mbox{ for all $i$}$$
and $\|\tilA-\trA\| \le \kappa \|\trA\|$. Additionally if only the above column-wise bound holds we will say that $\tilA$ is $\delta$-close to $\trA$. 
\end{definition}

\noindent This is a natural measure to use, since we can only hope to learn the columns of $\trA$ up to relabeling and sign-flips. In our analysis, we will assume throughout that $\pi(\cdot)$ is the identity permutation and $\sigma(\cdot) \equiv +1$ because our family of generative models is invariant under this relabeling and it will simplify our notation. 

 Also throughout this section let $\sgn(\cdot)$ denote the coordinate-wise sign function and recall that $\eta$ is the learning rate, which we will set later. Also we fix  both $\delta, \delta_0 = O^*(1/\log n)$. We will also assume that in each iteration, our algorithm is given a fresh set of $p$ samples. Our main theorem is:

\begin{theorem}\label{thm:simplestupdate}
Suppose that $\tilA^0$ is $(2\delta,2)$-\near to $\trA$ and that
$\eta = \Theta(m/k)$. Then if each update step in Algorithm~\ref{eqn:simplestupdate} uses $p = \widetilde{\Omega}(mk)$ fresh samples, we have
$$\Exp[\|\tilA_i^s - \trA\|^2]\le (1-\tau)^s \|\tilA^0_i - \trA_i\|^2 + O(k^2/n^2)$$
for some $0 < \tau < 1/2$ and for any $s=1,2, ... , T$. In particular it converges to $\trA$ geometrically with systemic error $O(k^2/n^2)$. 
\end{theorem}
\Tnote{Reminder: address the defintion of systemic error (probably in Section 2)}
%\Rnote{Made the main theorem technically correct. It still feels incomplete as a main theorem though.}


Our strategy is to prove that $\hat{g}^s$ is $(\alpha,\beta,\epsilon)$-correlated (see Definition~\ref{eqn:con}) with the desired solution $\trA$, and then to prove that $\| \tilA\|$ never gets too large. We will first prove that if $\tilA$ is somewhat close to $\trA$ then the estimate $\tilx$ for the representation almost always has the correct support. Here and elsewhere in the paper, we use ``very high probability"  to mean that an event happens with probability at least $1- 1/n^{\omega(1)}$. 

\begin{lemma}\label{lem:sign-correct}
Suppose that $\tilA^s$ is $\delta$-close to $\trA$.  Then
$$\mbox{{\em sgn}}(\mbox{{\em threshold}}_{C/2}((\tilA^s)^Ty)  ) = \mbox{{\em sgn}}(\trx)$$ with very high probability over the choice of the random sample $y = \trA\trx$.
\end{lemma}

\noindent We defer the proof of this lemma to Section~\ref{subsec:support}; in fact this lemma will be the first step in analyzing all of the update rules we consider in this paper. However this is just one step on the way towards proving that $\hat{g}^s$ is correlated with the true solution. 


\begin{algorithm}\caption{Neurally Plausible Update Rule}\label{eqn:simplestupdate}
\vspace{0.1in}
\textbf{Initialize} $\tilA^0$ that is $(\delta_0, 2)$-near to $\trA$

\textbf{Repeat}  for $s = 0, 1, ..., T$
\vspace{-0.1in}
\begin{align*}
\textbf{\textbf{Decode: }} & \tilx^{(i)} = \textrm{threshold}_{C/2}((\tilA^s)^Ty^{(i)})  \textrm{ for $i = 1, 2, ... , p$}\nonumber\\
\textbf{\textbf{Update: }} & \tilA^{s+1} = \tilA^s - \eta \hat{g}^{s} \mbox{ where } \hat{g}^{s} = \frac{1}{p}\cdot\sum_{i=1}^p (y^{(i)} - \tilA^s \tilx^{(i)}) \sgn(\tilx^{(i)})^T \nonumber
\end{align*}
\end{algorithm}

The next step in our proof is to use the properties of the generative model to derive a new formula for $\hat{g}^s$ that is more amenable to analysis. %For simplicity, we start from the case when we are given infinite number of samples at each iteration. And 
We define $g^s$ to be the expectation of $\hat{g}^s$
\begin{eqnarray}
g^s := \Exp[\hat{g}^s] = \Exp[(y - A^s \wtilx) \sgn(\tilx)^T]
\end{eqnarray}
where random variable $x := \textrm{threshold}_{C/2}((\tilA^s)^Ty)$ is the decoding of $y$. 
Let $q_i = \Pr[\trx_i\ne 0]$ and $q_{i,j} = \Pr[\trx_i\trx_j\ne 0]$, and define $p_i = \E[\trx_i\sgn(\trx_i)|\trx_i\ne 0]$. 

 Here and in the rest of the section,  we will let $\gamma$ denote any vector whose norm is negligible (i.e. smaller than $1/n^C$ for any large constant $C > 1$).

\begin{lemma}\label{lem:OF-simplified-update}
Suppose that $\tilA^s$ is $(2\delta,2)$-\near to $\trA$. Then the update step in Algorithm~\ref{eqn:simplestupdate} takes the form 
$$\Exp[\tilA_i^{s+1}] = \tilA_i^{s} - \eta g_i^s$$
where $g_i^s = p_iq_i \left(\lambda^s_i\tilA_i^s - \trA_i +\epsilon^s_i \pm \gamma\right)$,  and $\lambda^s_i = \langle \tilA_i^s, \trA_i\rangle $ and
$$\epsilon_i^s = \Big( \tilA^s_{-i} \mbox{diag}(q_{i,j}) \left(\tilA_{-i}^s\right)^T \Big)\trA_i/q_i$$
Moreover the norm of $\epsilon^s_i$ can be bounded as $\|\epsilon^s_i\|\le O(k/n)$. 
\end{lemma}

\begin{proof}  
Since $\tilA^s$ is $(2\delta,2)$-\near to $\trA$, $\tilA^s$ is $2\delta$-close to $\trA$. We can now invoke Lemma~\ref{lem:sign-correct} and conclude that with high probability, $\sgn(\trx) = \sgn(\tilx)$.
Let $\calF_{\trx}$ be the event that $\sgn(\trx) = \sgn(\tilx)$, and let $\mathbf{1}_{\calF_{\trx}}$ be the indicator function of this event. 

To avoid the overwhelming number of appearances of the superscripts, let $B = \tilA^s$ throughout this proof. Then we can write $g_i^s$ as 
\begin{eqnarray*}
g_i^s &=&  \E[(y - B \wtilx) \sgn(\tilx_i)] 
\end{eqnarray*}

\noindent Using the fact that $\mathbf{1}_{\calF_{\trx}} + \mathbf{1}_{\bar{\calF}_{\trx}} = 1$ and that $\calF_{\trx}$ happens with  very high probability:
\begin{eqnarray}
g_i^s &=&  \E[(y - B \wtilx) \sgn(\tilx_i) \mathbf{1}_{\calF_{\trx}}] +   \E[(y - B \wtilx) \sgn(\tilx_i)  \mathbf{1}_{\overline{\calF}_{\trx}}] \nonumber \\
&=& \E[(y - B \wtilx) \sgn(\tilx_i)  \mathbf{1}_{\calF_{\trx}}] \pm \gamma \label{eqn:g_s1}
\end{eqnarray}

The key is that this allows us to essentially replace $\sgn(\tilx)$ with $\sgn(\trx)$. Moreover,  let $S= \mbox{supp}(\trx)$. Note that when $\calF_{\trx}$ happens $S$ is also the support of $\tilx$. Recall that according to the decoding rule (where we have replaced $\tilA^s$ by $B$ for notational simplicity) $\tilx = \textrm{threshold}_{C/2}(B^T y)$. Therefore, $\tilx_S = (B^Ty)_S = B_S^T y = B_S^T\trA \trx$. Using the fact that the support of $\tilx$ is $S$ again, we have $B\tilx = B_S^TB_S\trA \trx$. Plugging it into equation (\ref{eqn:g_s1}):
\begin{eqnarray*}
g_i^s &=& \E[(y - B \tilx) \sgn(\tilx_i) \mathbf{1}_{\calF_{\trx}}] \pm \gamma\\
 &=& \E[(I - B_S B_S^T ) \trA \trx\cdot  \sgn(\trx_i)  \mathbf{1}_{\calF_{\trx}}] \pm \gamma\\
&=& \E[(I - B_S B_S^T ) \trA \trx \cdot \sgn(\trx_i)  ]  - \E[(I - B_S B_S^T ) \trA \trx \cdot \sgn(\tilx_i) \mathbf{1}_{\bar{\calF}_{\trx}}] \pm \gamma\\
&=& \E[(I - B_S B_S^T ) \trA x\cdot \sgn(\trx_i) ]   + 2\gamma
\end{eqnarray*}
where again we have used the fact that $\calF_{\trx}$ happens with very high probability. Now we rewrite the expectation above using subconditioning where we first choose the support $S$ of $\trx$, and then we choose the nonzero values $\trx_S$. 
\begin{eqnarray*}
\E[(I - B_S B_S^T ) \trA \trx \cdot \sgn(\trx_i) ]  &=& \E_S \Big[ \E_{\trx_S}[(I - B_S B_S^T ) \trA \trx \cdot \sgn(\trx_i) | S ] \Big] \\
&=& \E [p_i (I - B_S B_S^T ) \trA_i\cdot  \sgn(\trx_i) ]
\end{eqnarray*}
where we use the fact that $\E[\trx_i \cdot \sgn(\trx_i) | S] = p_i$. Let $R = S -\{i\}$. Using the fact that $B_SB_S^T  = B_iB_i^T + B_RB_R^T$, we can split the quantity above into two parts, 
\begin{eqnarray*}
g_i^s &=& p_i \E[(I - B_i \tilA_i^T) \sgn(\trx_i)] \trA_i + p_i \E[(I - B_R \tilA_R^T) \sgn(\trx_i)] \trA_i \\
&=& p_iq_i \Big(I - B_i B_i^T\Big)\trA_i +  p_i \Big( B_{-i} \mbox{diag}(q_{i,j}) B_{-i}^T \Big)\trA_i \pm \gamma.
\end{eqnarray*}

\noindent where $\mbox{diag}(q_{i,j})$ is a $m\times m$ diagonal matrix whose $(j,j)$-th entry is equal to $q_{i,j}$, and $B_{-i}$ is the matrix obtained by zeroing out the $i$th column of $B$. Here we used the fact that $\Pr[i\in S] = q_i$ and $\Pr[i,j\in S] = q_{ij}$. 

Now we set $B = \tilA^s$, and rearranging the terms, we have 
$$g_i^s = p_iq_i \left(\langle \tilA_i^s, \trA_i\rangle\tilA_i^s - \trA_i +\epsilon^s_i \pm \gamma\right)$$ 
where $\epsilon_i^s = \Big( \tilA^s_{-i} \mbox{diag}(q_{i,j}) \left(\tilA_{-i}^s\right)^T \Big)\trA_i/q_i$, which can be bounded as follows
$$\|\epsilon_i^s\|\le \|\tilA^s_{-i}\|^2 \max_{j\neq i} q_{i,j}/q_i \le O(k/m) \|\tilA^s\|^2 = O(k/n)$$
where the last step used the fact that  $\frac{\max_{i\neq j}q_{i,j}}{\min q_i } \le O(k/m)$, which is an assumption of our generative model.  
\end{proof}

\noindent In particular, $p_iq_i$ is a scaling constant and $\lambda_i \approx 1$, therefore from the above formula we should expect that $g_i^s$ is well-correlated with $\tilA_i^s - \trA_i$. 


In Section~\ref{sec:hypothesis} we prove various auxiliary lemmas we need in order to fit into the framework we developed in the previous section. In particular, in Section~\ref{sec:progress}, we prove that if $\tilA^s$ is $(2\delta,2)$-\near to $\trA$ then $g_i^s$ is indeed $(\alpha,\beta,\epsilon)$-correlated with $A_i$ (Lemma~\ref{cor:one-step}). Finally we prove that if $\tilA^s$ is $(2\delta,2)$-\near to $\trA$ then $\|\tilA^{s+1} - \trA\|\le 2\|\trA\|$ (Lemma~\ref{lem:nowhiten}). By a simple induction, these two Lemmas with Theorem~\ref{thm:tiger-convergence} imply Theorem~\ref{thm:simplestupdate-infinitesample}, the simplified version of Theorem~\ref{thm:simplestupdate} with the number of samples $p$ accessed at each iteration being infinite. Theorem~\ref{thm:simplestupdate} with finite sample complexity bound is then proved in , Section~\ref{sec:sample_complexity}, by essentially bounding the fluctuation of $\hat{g}^s$ around $g^s$. %This yields our main theorem. 
%
%In Section~\ref{sec:hypothesis} we complete the proof of our main theorem by proving various auxiliary lemmas we need in order to fit into the framework we developed in the previous section. In particular, in Section~\ref{sec:progress}, we prove that if $\tilA^s$ is $(2\delta,2)$-\near to $\trA$ then $g_i^s$ is indeed $(\alpha,\beta,\epsilon)$-correlated with $A_i$ (Lemma~\ref{lem:checking_condtion1}). Finally we prove that if $\tilA^s$ is $(2\delta,2)$-\near to $\trA$ then $\|\tilA^{s+1} - \trA\|\le 2\|\trA\|$ (Lemma~\ref{lem:nowhiten}). This yields our main theorem. 

%\Tnote{This only proves the infinite samples version of the Theorem}
 %that Algorithm~\ref{eqn:simplestupdate} converges to a globally optimal solution. In particular when we set $\eta = O(m/k)$ the algorithm converges to a point that has systematic bias $O(\epsilon/\alpha) = O(k/n)$. This yields our main theorem, that the neurally plausible update rule introduced at the beginning of this section converges to a globally optimal code under the distributional assumptions of our generative model.













%\subsection{Old draft}
%\input{indicatorinclude_old}

==> introflat.tex <==

\section{Introduction}

 {\em Sparse} representations are believed to be an essential feature of neural coding of information: 
  information is carried by a small subset of active neurons, which is energy efficient. % from a biological level. 
  Other reasons in support of such representations come from linked fields: in signal processing natural signals turn out to be sparse in an appropriately chosen basis, and in machine learning,  imposing a sparsity constraint on the representation helps avoid {\em over-fitting}. The seminal work of Olshausen and Field~\cite{OF} showed that
  a sparse coding algorithm applied to a collection of natural images recovers wavelet-like filters that resemble the receptive fields of cells in the
  visual cortex. Based on biological considerations, their work introduced the  {\em linear model} for sparse coding: 
given a dataset $y^{(1)}, y^{(2)}, \ldots, y^{(p)}$ of $n$-dimensional vectors, %\in \mathbb{R}^n$, 
find a  set of basis vectors $A_1, A_2, \ldots, A_m$ (sometimes called a {\em dictionary})
and {\em sparse} coefficient vectors $x^{(1)}, x^{(2)}, \ldots, x^{(p)} \in \mathbb{R}^m$ such that
$\sum_{j =1}^m x^{(i)}_jA_j$ well-approximates each $y^{(i)}.$
%the {\em reconstruction error} $\sum_{i=1}^p \| y^{(i)} - \sum_{j =1}^m x^{(i)}_jA_j\|_2.$
 % is  {\em sparse coding}: %which is the focus of our paper.
The number of basis vectors $m$ usually exceeds the dimension $n$. This is called the {\em overcomplete} case and permits more flexible and 
robust representations, and $m/n$ in neural encodings is estimated to be as large as $500$~\cite{}. % seem  high as $500$~\cite{.}
%is also the interesting one in neuroscience. 
%\Tnote{Shall we say a few words about what is the physical meaning of these notations in OF? (like $y$ is a picture, and $x$ is the activation of the neurons, and $A$ is the weights on synapses? ) OF uses quite different notations and the data in OF is a matrix, though we linearize it}

% Is is estimated that the human visual cortex is overcomplete by a factor 
%of a few hundred.    

%In matrix notation, the above error is represented as $\sum_{i=1}^p \| y^{(i)} - A x^{(i)}\|_2$, where 
Denoting the $n\times m$ matrix of basis vectors as $A$,
%is the
%$n\times m$ matrix whose $j$th column is $A_j$. Thus 
sparse coding is a 
nonconvex optimization problem of the form
\begin{equation} \min_{A, x^{(1)},\ldots, x^{(p)}}\quad \sum_{i=1}^p \|y^{(i)} - A x^{(i)}\|_2 + \sum_{i=1}^p\ell(x^{(i)}),
\label{eqn:energyfn} \end{equation}
where  $\ell(\cdot)$ is a nonlinear penalty function that encourages sparsity. 
%Many natural choices for this function empirically seem to give qualitatively similar results~\cite{OF}. 
This paper assumes a {\em hard} penalty function that restricts the coefficient vectors to have at most $k$ non-zeros\footnote{In particular, $\ell(x)$ is zero if $x$ has at most $k$ non-zeros and otherwise is infinite.}. 
Though usually believed %believed to be computationally 
to be computationally harder than the {\em soft} sparsity constraints used in \cite{OF} (which allow many small nonzero entries in $x^{(i)}$), it
 has been shown to yield bases that are more biologically realistic~\cite{rehsommer}.

%\Anote{We do not use the $\ell$ penalty function anywhere in the paper. Why are we using this notation? if it is to emphasize that it is a non %convex optimization problem, then we could just choose a particular $\ell$, namely the one that puts infinite penalty on $x_i$'s with more %than $k$ non-zeros, and no penalty on everything else. Also this notation $x_i$ is inconsistent with the notation we use later in the paper. %Should we make it $x^{(i)}$?}

The optimization in (\ref{eqn:energyfn}) has no known {\em efficient} algorithm, in other words one that 
{\em always} finds the optimum  in time that is some polynomial function of $m, n$ and $k$. (Thus $m^2n k$ is efficient whereas $m^k$ is not.)
Of course, no efficient algorithms are known for the non-convex optimization problems that arise in a variety of other domains as well. Computational complexity
suggests an explanation since such algorithms do not exist if $P \neq NP$~\cite{AroraBarak}. In practice 
such problems are solved --- also in~\cite{OF} --- via some adaptation of gradient descent. Although this
 could in principle get trapped in local optima, Olshausen and Field as well as subsequent researchers
 have shown
empirically that neural algorithms for sparse coding yield reasonable bases. % that are biologically plausible. 
%  hence they do not necessarily find a basis that enables a sparse representation, even if one exists. 
Such empirical success begs for a theoretical explanation: Is it possible to give a rigorous analysis of 
gradient descent --- more broadly, of neural computation --- instead of relying solely on empirical evidence? 
%Concretely, can we prove that the algorithm quickly arrives at the global optimum while avoiding local optima?
If possible, such a proof would not only yield new insight but could also  
suggest promising new algorithms for variants of these problems in machine learning and signal processing. 
This paper will suggest that such mathematical rigor is indeed possible for sparse coding,
with some careful formulation of the problem.
% to overcoming this hurdle.
% is the main goal of the current paper. 
%\Tnote{I thought ``biologically plausibility'' usually refers to the algorithm but not the solution that is obtained from the algorithm.  }

 %Computational complexity \cite{AroraBarak} suggests that efficient solution of nonconvex optimization problems on 
%{ \em all} problem instances is likely to be impossible (with {\em any} algorithm, not just gradient descent) since such an algorithm would imply $P = NP$. % \footnote{Many non-convex problems are NP-hard, implying they are unlikely to have any efficient algorithms at all, let alone
% ones relying on gradient descent.}, 
Since nonconvex optimization seems hopeless in general, a rigorous analysis must assume a {\em class} of natural instances motivated by applications. Here we assume a generative model (detailed below) for the data whereby each $y^{(i)}$ is generated as
 $$y^{(i)} = \trA \trxs{j} + \xi$$ where $\trxs{1}, \trxs{2}, \ldots, \trxs{p}$  are iid samples from a well-behaved distribution, $\xi$ is a noise vector, and the code matrix $\trA$ is suitably well-behaved to produce unique and robust encodings (namely, if $x, x'$ are very different then so are $\trA x$ and $\trA x'$).
 %Moreover $A$ is {\em incoherent} --- its columns are uncorrelated with each other (see Section~\ref{sec:notations} for details). These %features ensure that 
 %so that the target representation is both unique and robust and 
 Standard statistical arguments show that
 the optimum solution to (\ref{eqn:energyfn}) is then essentially unique given enough samples. Note however that this does not rule out the existence of many local optima that could trap gradient descent and prevent it from ever reaching the global optimum. 

%Focusing on a natural subclass can help confront two confounding issues: $(1)$ the sparse representation could be nonunique in the target basis: $A x \approx Ax'$ for two very different sparse vectors $x$ and $x'$; and $(2)$ the dataset is degenerate: some basis vectors rarely get used in the optimum sparse code. These issues can be sidestepped in a standard way by assuming a generative model for the data, whereby each $y^{(i)}$ is assumed to be generated as
% $y^{(i)} = A x^{(i)} + \eta$ where $A$ is some fixed and well-behaved matrix ("ground truth basis") and $x^{(1)}, x^{(2)}, \ldots,$  are iid samples from a well-behaved distribution, and $\eta$ is a noise vector (see Section~\ref{sec:notations} for details). 

Some very recent work~\cite{SWW, AAJNT, AGM} has yielded efficient algorithms that {\em provably} solve sparse coding in the above generative model
with high probability. Unfortunately, these  require batch processing and some complex manipulations that are not necessarily available in biological systems. The important result in this paper is that it is possible to rigorously analyze a class of natural {\em neurally plausible}\footnote{{\em neural plausibility} is often not precisely defined in computational neuroscience. Here it refers to an algorithm that encodes its current estimate $\tilde{A}$ in a distributed manner as the weights of neural edges and whose updates involve sums and thresholds of values from neighboring neurons.} algorithms --- including the original algorithms of \cite{OF} --- for sparse coding, which use simple operations such as matrix multiplication and thresholding. A side benefit is that
these simpler algorithms also happen to be much more efficient --- both in sample complexity and running time --- than all previously known algorithms. 

Iterative algorithms for minimizing non-convex functions are notoriously difficult to analyze, and the approach of \cite{OF} is no exception. Our key insight is to view it instead as attempting to minimize an {\em unknown} convex function given an approximation to its gradient; this view is derived by taking advantage of the generative model. Moreover, we introduce a general framework that allows analysis of several variations of the algorithm, and may be useful in other settings in the future. There have been several prior attempts to analyze iterative algorithms for sparse coding, but ours is the first that works under weak assumptions about the initial estimate where the objective function cannot be well-approximated by a  convex function. 

%The key idea is to relate the gradient descent on the nonconvex energy function to the gradient of a related but unknown {\em convex} function.
%To analyse such situations, a general and formal framework is introduced % (see Appendix). This framework 
%that allows  analysis of several variations of the algorithm, and may be useful in other settings in future.


% However, recently new algorithms ---complicated ones, not gradient descent--- were described for recovering this ground truth and optimum solution~\cite{. }. The new result in the current paper is that even natural neural algorithms can recover such a dictionary, and more efficiently than these recent algorithms. 
% for
%  $(a)$ $A$ is $\mu$ incoherent \-- i.e. $|\langle A_i,A_j \rangle | \leq \mu/\sqrt{n}$ for each pair of columns; this is well-known to avoid %the first problem~\cite{Donoho}. $(b)$ Each $x_i$ is an i.i.d. sample from a suitable distribution as described in Section~\ref{sec:notations} %and $(c)$ $A$ has bounded operator norm \-- i.e. $\|A\| \leq \sqrt{m/n}$


%\Snote{Need a para here comparing this algorithm's performance with those of recent papers.}

\iffalse 
\paragraph{Proof Overview:} 
The approach taken by Olshausen and Field is to perform gradient descent on the nonconvex energy function given in (\ref{eqn:energyfn}). However our understanding of these types of algorithms is limited to showing that they make progress in each step but can get stuck in local optima. Nevertheless, in both simulations and on real data they seem to find good solutions under quite general conditions. Can we establish provable guarantees for the approach of Olshausen and Field (and related neurally plausible algorithms) in the right model? 

Our main new insight is to view these algorithms as attempting to minimize an {\em unknown} convex function given an approximation to its gradient. This suggests an interesting, new set of questions, whereby tools from optimization could lead to faster and more sample efficient algorithms for sparse coding and other related problems. This may be reminiscent
of {\em stochastic gradient descent},
a popular technique for convex programming  that involves moving along a randomly chosen direction whose {\em expectation} is the gradient.
In our setting the direction of movement is indeed stochastic (since $y^{(i)}$'s in (\ref{eqn:energyfn}) are iid from some underlying
distribution) but the expectation is not the true gradient --- there is {\em systematic} error because $A \neq \tilde{A}$. 

We give a general methodology to control the error, whereby we can plug in various update rules and analyze their convergence. The highlights of this method are that we obtain $(a)$ the first neurally plausible algorithm with provable guarantees for sparse coding, that converges to a globally optimal solution $(b)$ the first algorithms whose running time is a fixed polynomial even as we approach the threshold for sparse recovery in incoherent dictionaries and $(c)$ the first algorithm for sparse coding with near optimal sample complexity. There have been a number of attempts to analyze simple update rules for sparse coding in the past, but the critical distinction is that our results hold when we initialize our methods from weak starting conditions where the columns of our current estimate $\tilde{A}$ are $1/\mbox{polylog}(n)$-close to the columns of $A$. In contrast, existing work assumes that the columns are$1/\mbox{poly}(n)$ close in which case the nonlinear energy function in (\ref{eqn:energyfn}) is essentially convex in the region we are optimizing over. Lastly, we complement our results with a simple initialization procedure. 

\fi
%The OF-style algorithm iteratively improves its estimate $\widetilde{A}$ for the optimum $A$. It wishes to move along the gradient of (\ref{eqn:energyfn}), but the gradient computation would require knowing each $x^{(i)}$. So the algorithm computes {\em estimates} of  each $x^{(i)}$ by trying to solve (exactly or approximately) for $z$ in 
%\begin{equation} \min \| y^{(i)} - \tilde{A} z\|. \label{eqn:localcompute}
%\end{equation} It uses these estimates to compute an estimate for the best improvement
%direction for $\widetilde{A}$.  The difficulty is that the estimates of $x^{(i)}$ yielded by (\ref{eqn:localcompute}) are highly suspect since the current $\widetilde{A}$ may be too inaccurate. Thus the iteration may end up moving $\widetilde{A}$ {\em away} from $A$ instead of {\em towards} it.
%may not approach $A$, or even move away.

%The main insight in our proof that this doesn't happen much is to link the nonconvex program (\ref{eqn:energyfn}) with a natural {\em convex} program: the one obtained from (\ref{eqn:energyfn}) by treating $x^{(i)}$'s as known. OF-style gradient descent for (\ref{eqn:energyfn}) can be viewed as an attempt to move in a direction that is an {\em estimate} for the gradient for this convex program (see Section~\ref{sec:OFframework}). This may be reminiscentof {\em stochastic gradient descent},a popular technique for convex programming  that involves moving along a randomly chosen direction whose {\em expectation} is the gradient. In our setting the direction of movement is indeed stochastic (since $y^{(i)}$'s in (\ref{eqn:localcompute}) are iid from some underlying distribution) but the expectation is not the true gradient ---there is {\em systematic} error because $A \neq \widetilde{A}$. The proof has to quantify and control this systematic error to show that it steadily decreases, in turn implying that $\widetilde{A} \rightarrow A$. This convergence proof can be presented in a formal framework similar to convex optimization, which appears in Section~\ref{sec:framework} and may be useful in other settings as well. 

%The above local improvement needs to be appropriately initialized as described in Section~\ref{??}. 
%This initialization uses computations of top singular vector of some matrix and is also neurally implementable.


%\Rnote{I think we need to be more precise here. The algorithm is only ``completely new'' comparing to our previous works. The algorithm is not very different from Olshausen and Field.}

%\Anote{Should we offer a definition of neural plausibility here, even though there is no precise one in the literature?}

%Firstly, one needs a well-posed problem whose  global
%optimum is unique and where the sparse representation is robust. 
%In principle we could be worried about the following issues confounding an algorithm:
%(1) The sparse representation is not unique if for example $A x \approx Ax'$ for two very different sparse vectors $x$ and $x'$.  
%There is a rich body of literature in statistics that identifies conditions which rule out the above scenario, such as when
%$A$ has the {\em restricted isometry property} or when $A$ is {\em incoherent}. 
%(2) The dataset is somehow degenerate and more than one basis matrix $A$ can minimize the cost function. %~(\ref{eqn:energyfn}).
%The natural way to sidestep this problem is to assume a generative model for the dataset whereby the 
%$x$ vectors are iid samples from some distribution and the each datapoint is generated according to
%$y = A \cdot x + \eta$, where $\eta$ is a gaussian noise vector and $A$ is the (fixed but unknown) basis matrix. 
%Then the best $A$ is unique with high probability. 

%Accordingly let's assume such a generative model from now on and that (a) $A$ is $\mu$-incoherent\footnote{The survey
%of Elad~\cite{} describes why incoherence is a natural condition in such cases.}, that is,
%$|<A_i,A_j>| \leq \mu/\sqrt{n}$ for each two columns $i, j$.  (b) The $x$'s are iid samples from a suitable distribution, as described in Section~\ref{}. 
%Furthermore we make the assumption (c) $A$ has low matrix norm $|A|_2 \leq ??$.

%Although assumptions (a), (b) suffice to ensure {\em uniqueness} of the global optima, they do not suffice to
%rule out local optima which may trap the continuous optimization. Such local optima can involve basis vectors
%that have nonnegligible components in some common low-dimensional subspace (see Appendix A), and assumption (c)
%turns out to rule them out.  Note that conditions (a) and (c) both speak to the intuition that the basis vectors
%should be "uncorrelated" or "almost orthogonal."

%Surprisingly, condition (c) doesn't appear necessary if one is willing to settle for algorithms that are  efficient on a computer but not necessarily neurally plausible. Such algorithms can use batch processing of inputs and arbitrary matrix computations, and
%were given recently in \cite{}.
%By contrast, neurally plausible algorithms should "store" $A$ in a single place and access it in very restricted ways (eg, via
%matrix-vector product with fresh data samples), and update it in an online fashion as more samples arrive. The neurally plausible algorithm in the current paper is completely new and not an adaptation of the earlier nonneural algorithms ---for example it is more
%efficient with respect to sample complexity and running time. 

==> modelflat.tex <==
%\section{Preliminaries}
%\label{sec:notations}

%Here we introduce the model that we will study in this paper, and provide some justification for it. 



% We will also standard notation for vectors and matrices. 
\iffalse 
For a vector $v$  $\|v\|$ denote its $\ell_2$ norm and for a matrix $A$ let $A_i$ denote its $i$th column. We will not be interested in the rows of matrices, so we reserve the notation $\tilde{A}^s$ to denote the value of the estimate $\tilde{A}$ in the $s$th iteration. % and let $A^j$ denote its $j$th row. 
Let $\|A\|$ denote its operator norm and let $\|A\|_F$ denote its Frobenius norm. Additionally let $\sgn(x)$ be the function that maps positive numbers to $1$, negative numbers to $-1$ and maps $0$ to $0$. We will apply $\sgn$ to vectors in which case we mean the entry-wise application of it. Also, let $\E_x[f(x)]$  denote the expectation of $f(x)$ with respect to the random variable $x$. We will omit the subscript when the random variable we are taking the expectation over is clear from context. Finally, let $\mathbf{1}_{\mathcal{A}}$ denote the indicator function of event $\mathcal{A}$.
\fi
\paragraph{The Generative Model.}
Lewicki and Sejnowski~\cite{LS} placed the Olshausen-Field work in a familiar statistical framework: data is assumed to be drawn from a generative model where data is generated as $y = \trA \trx + \xi$ where $\xi$ is a noise vector and $\trx$ is drawn from an unknown distribution $\mathcal{D}$ 
Recovery of $A, x$ seeks to maximise likelihood --- perhaps heuristically, with no guarantees of quick convergence. We follow this standard statistical framework, but using provably efficient estimators.

The generative model must make more assumptions about $\trA$ to restrict attention to code matrices that yield robust and well-behaved representations in the first place. This issue was well-studied in {\em sparse recovery} in recent years (see~\cite{E} for background).
 We assume that $\trA$ is {\em incoherent}, which
formalizes the intuition that column vectors are fairly distinct: formally, if each column is a unit vector then $|\langle \trA_i,\trA_j \rangle | \leq \mu/\sqrt{n}$ for each distinct $i, j$.
%the ). We will
We also require that the operator norm of $\trA$ (maximum $\ell_2$ norm of a linear combination of columns involving a unit coefficient vector) is appropriately bounded: $\|\trA\| = O(\sqrt{m/n})$.  These conditions are satisfied by a rich family of codes, such as randomly generated ones as well as concatenations of various families of wavelets \cite{DE}.

It is typical to assume a special functional form for the distribution $\mathcal{D}$ for the unknown $\trxs{i}$. 
Our analysis allows any distribution satisfying the following conditions, which are motivated by the general intuition (and original motivation of \cite{OF}) that 
a good choice for a sparse coding matrix is one makes coordinates of $\trx$'s fairly independent: 
  $(a)$ the support $S = \mbox{supp}(\trx)$ has at most $k$ elements and $\Pr[i\in S] \approx k/m$ and $\Pr[i,j\in S] \approx k^2/m^2$; $(b)$ the distribution is normalized so that $\E[\trx_i|\trx_i\ne 0] = 0$; $\E[{\trx_i}^2|\trx_i\ne 0] = 1$ and when $\trx_i\ne 0$, $|\trx_i|\ge C$ for an arbitrary constant $C \le 1$ and $(c)$ the non-zero entries are pairwise independent and subgaussian, conditioned on the support. We will be able to tolerate noise whose magnitude is almost as large as that of the signal, and in fact many of the above conditions can be further relaxed if one reduces the allowed sparsity $k$. 

\paragraph{Notation.}
As is customary in the analysis of algorithms, asymptotic notation is used: $O(f(n))$ denotes a function upper bounded by $C f(n)$ for some large enough constant $C$ for any $n \geq n_0$;  $O^*(f(n))$ denotes a function that is upper bounded by $C f(n)$ for some small enough constant $C$. 
 Likewise, $\Omega(f(n))$ denotes a function lower bounded by $C f(n)$ for some small enough constant $C$ for any $n \geq n_0$ and $\Omega^*(f(n))$ denotes a function that is lower bounded by $C f(n)$ for a large enough constant $C$. 
 







==> newinitinclude.tex <==

\section{Further Applications}
\label{sec:otherrules}

Here we apply our framework to design and analyze further variants of alternating minimization. 

\subsection{Revisiting Olshausen-Field}

In this subsection we analyze a variant of the Olshausen and Field update rule. This update rule corresponds directly to taking the gradient of the energy function described in Section~\ref{sec:schema}. However there are quadratic error terms that arise in the expressions we derive for $g^s$ and bounding them is more challenging. We will also need to make (slightly) stronger assumptions on the distributional model, and in addition to assuming that $q_i \approx k/m$ and $q_{i,j} \approx k^2/m^2$ we will also need to assume that for distinct $i_1,i_2,i_3$ we have $q_{i_1,i_2,i_3} = O(k^3/m^3)$ where $q_{i_1,i_2,i_3} =  \Pr[i_1,i_2,i_3\in S]$. As in previous sections, we fix both $\delta, \delta_0 = O^*(1/\log n)$. 


%the update rule that directly corresponds to taking the gradient of energy function at the decoding $\tilx$. Let $\tilx = \mbox{threshold}_{C/2}(\tilA^T y)$ be the decoding, this rule moves $\tilA$ along direction $\nabla_{\tilA} \mathcal{E}(\tilA, \tilx)$. This is very similar to the procedure used in \cite{OF}, except they use a more complicated decoding algorithm.




%We will first show that the update direction $g^s$  in this rule is also $(\alpha, \beta, \epsilon)$-correlated with the true answer $\trA$ if the current estimate $\tilA^s$ is $(2\delta,2)$-\near to $\trA$. However, unlike the previous update, it is not clear whether this rule preserves nearness. In order to handle this problem we need to change the problem into a constrained optimization problem, and enforce the nearness constraints.

%Also, in order to analyze this rule we need stronger assumptions on the distribution of the support of $x$: let $q_{i_1,i_2,i_3} =  \Pr[i_1,i_2,i_3\in S]$, then when $i_1,i_2,i_3$ are distinct we have $q_{i_1,i_2,i_3} = O(k^3/m^3)$ (recall previously we only required the pairwise marginals to be close to $k^2/m^2$). In the rest of the subsection we are going to prove the following theorem:

Recall that we have chosen to work with the measure of closeness given in Definition~\ref{def:near}. Our main theorem in this subsection is:

\begin{theorem}\label{thm:OFupdate}
Suppose that $\tilA^0$ is $(2\delta,2)$-\near to $\trA$ and that
$\eta = \Theta(m/k)$. Then in Algorithm~\ref{eqn:ofrule}, at each step $s$, 
%Then if each update step in Algorithm~\ref{eqn:ofrule} uses $p = \widetilde{\Omega}(mk)$ fresh samples, 
we have for each column $i$, 
$$\|\tilA_i^s - \trA_i\|^2\le (1-\tau)^s \|\tilA^0_i - \trA_i\|^2 + O(k^2/n^2)$$
for some $0 < \tau < 1/2$ and for any $s=1,2, ... , T$. In particular it converges to $\trA$ geometrically with systemic error $O(k^2/n^2)$. 
\end{theorem}

%\Tnote{systemic squared error}
%\Tnote{Need $\Exp$ in LHS if with finite number of samples}
Note that in Algorithm~\ref{eqn:ofrule} (and Algorithm~\ref{eqn:nonoiserule} in the next section), we use the expectation of the gradient over the samples instead of the empirical average. We can actually show that the sample complexity of estimating the expectation $g^s$ in Algorithm~\ref{eqn:ofrule} and Algorithm~\ref{eqn:nonoiserule} is also $\widetilde{\Omega}(mk)$, similar to that of Algorithm~\ref{eqn:simplestupdate}, though the proofs are simply redundant repetitions of that of Theorem~\ref{thm:simplestupdate}. Thus we omit them and stick to the infinite number case which captures most of difficulties.   
%\subsection{Making Progress}


Our first goal is to prove that (this time for Algorithm~\ref{eqn:ofrule}) each column of $g^s$ is $(\alpha,\beta,\epsilon)$-correlated with $\trA_i$. The main step is to prove an analogue of Lemma~\ref{lem:OF-simplified-update} that holds for the new update rule. For simplicity, we also 

\begin{lemma}\label{lem:OFupdate}
Suppose that $\tilA^s$ is $(2\delta,5)$-\near to $\trA$ Then each column of $g^s$ in Algorithm~\ref{eqn:ofrule} takes the form
%$$\tilA_i^{s+1} = \tilA_i^s - \eta g_i^s,$$
%where 
$$g_i^s = q_i\left((\lambda_i^s)^2\tilA_i^s - \lambda_iA_i^s +\epsilon_i^s\right)$$
where $\lambda_i = \langle \tilA_i, \trA_i \rangle$.  Moreover the norm of $\epsilon_i^s$ can be bounded as $\|\epsilon_i^s\|\le O(k^2/mn)$. 
\end{lemma}

%\Tnote{This is only about infinite number of samples}
\begin{algorithm}\caption{Olshausen-Field Update Rule}\label{eqn:ofrule}
\vspace{0.1in}
\textbf{Initialize} $\tilA^0$ that is $(\delta_0, 2)$-near to $\trA$

\textbf{Repeat}  for $s = 0, 1, ..., T$
\vspace{-0.1in}
\begin{align*}
\textbf{\textbf{Decode: }} & \tilx = \textrm{threshold}_{C/2}((\tilA^s)^Ty)  \textrm{ for each sample $y$}\nonumber\\
%\textrm{ for $i = 1, 2, ... , p$}\nonumber\\
\textbf{\textbf{Update: }} & \tilA^{s+1} = \tilA^s - \eta g^{s} \mbox{ where } g^{s} = \Exp[(y - \tilA^s \tilx) \tilx^T] \quad \nonumber\\
%= \frac{1}{p}\sum_{i=1}^p (y^{(i)} - \tilA^s \tilx^{(i)}) (\tilx^{(i)})^T \quad \nonumber\\
\textbf{\textbf{Project: }}& \tilA^{s+1} = \mbox{Proj}_{\mathcal{B}} \tilA^{s+1} \mbox{(where $\mathcal{B}$ is defined in Definition~\ref{def:whiten})}\nonumber
\end{align*}
\end{algorithm}

\noindent We remark that unlike the statement of Lemma~\ref{lem:checking_condtion1}, here we will not explicitly state the functional form of $\epsilon_i^s$ because we will not need it. 

\begin{proof} 
The proof parallels that of Lemma~\ref{lem:OF-simplified-update}, although we will use slightly different conditioning arguments as needed. Again, we define $\mathcal{F}_{\trx}$ as the event that $\sgn(\trx) = \sgn(\tilx)$, and let $\mathbf{1}_{\calF_{\trx}}$ be the indicator function of this event. We can invoke Lemma~\ref{thm:supp} and conclude that this event happens with high probability. Moreover let $\mathcal{F}_i$ be the event that $i$ is in the set $S = \mbox{supp}(\trx)$ and let $\mathbf{1}_{\mathcal{F}_i}$ be its indicator function. 

When event $\mathcal{F}_{\trx}$ happens, the decoding satisfies $\tilx_S = \tilA_S^T \trA_S \trx_S$ and all the other entries are zero. Throughout this proof $s$ is fixed and so we will omit the superscript $s$ for notational convenience. We can now rewrite $g_i$ as 
\begin{eqnarray*}
g_i &=&  \E[(y - \tilA \tilx) \tilx^T] =  \E[(y - \tilA \tilx) \tilx_i^T  \mathbf{1}_{\calF_{\trx}}  ] +  \E[(y - \tilA \tilx) \tilx_i^T (1- \mathbf{1}_{\calF_{\trx}}) ]   \\
&=& \E\left[(I-\tilA_S^T\tilA_S)\trA_S\trx_S{\trx_S}^T{\trA_S}^T\tilA_i \mathbf{1}_{\calF_{\trx}} \mathbf{1}_{\mathcal{F}_i} \right]  \pm \gamma \\
&=& \E\left[(I-\tilA_S^T\tilA_S)\trA_S\trx_S{\trx_S}^T{\trA_S}^T\tilA_i \mathbf{1}_{\mathcal{F}_i} \right] \\
%&& \qquad - \E\left[(I-\tilA_S^T\tilA_S)\trA_S\trx_S{\trx_S}^T{\trA_S}^T\tilA_i (1 - \mathbf{1}_{\calF_{\trx}} ) \mathbf{1}_{\mathcal{F}_i} \right]  \pm \gamma \\
&=& \E\left[(I-\tilA_S^T\tilA_S)\trA_S\trx_S{\trx_S}^T{\trA_S}^T\tilA_i \mathbf{1}_{\mathcal{F}_i} \right]  \pm \gamma
\end{eqnarray*}

Once again our strategy is to rewrite the expectation above using  subconditioning where we first choose the support $S$ of $\trx$, and then we choose the nonzero values $\trx_S$. 
\begin{eqnarray*}
g_i &=& \E_S \Big[ \E_{\trx_S}[ (I-\tilA_S^T\tilA_S)\trA_S\trx_S{\trx_S}^T{\trA_S}^T\tilA_i \mathbf{1}_{\mathcal{F}_i} | S ] \Big] \pm \gamma \\
&=& \E\left[(I-\tilA_S\tilA_S^T)\trA_S{\trA_S}^T\tilA_i \mathbf{1}_{\mathcal{F}_i} \right] \pm \gamma\\
&=& \E\left[(I-\tilA_i\tilA_i^T - \tilA_R{\tilA_R}^T)(\trA_i{\trA_i}^T + \trA_R{\trA_R}^T)\tilA_i  \mathbf{1}_{\mathcal{F}_i} \right] \pm \gamma\\
&=& \E\left[(I-\tilA_i\tilA_i^T)(\trA_i{\trA_i}^T)\tilA_i  \mathbf{1}_{\mathcal{F}_i} \right]
+\E\left[(I-\tilA_i\tilA_i^T)\trA_R{\trA_R}^T\tilA_i  \mathbf{1}_{\mathcal{F}_i} \right]\\
&& \qquad - \E\left[\tilA_R{\tilA_R}^T \trA_i{\trA_i}^T\tilA_i \mathbf{1}_{\mathcal{F}_i} \right]
- \E\left[\tilA_R\tilA_R^T \trA_R {\trA_R}^T\tilA_i  \mathbf{1}_{\mathcal{F}_i} \right] \pm \gamma
\end{eqnarray*}

Next we will compute the expectation of each of the terms on the right hand side. This part of the proof will be somewhat more involved than the proof of Lemma~\ref{lem:OF-simplified-update}, because the terms above are quadratic instead of linear. The leading term is equal to $q_i (\lambda_i \trA_i - \lambda_i^2 \tilA_i)$ and the remaining terms contribute to $\epsilon_i$. The second term is equal to $(I-\tilA_i\tilA_i^T) \trA_{-i}\mbox{diag}(q_{i,j}){\trA_{-i}}^T \tilA_i$ which has spectral norm bounded by $O(k^2/mn)$. The third term is equal to $\lambda_i \tilA_{-i}\mbox{diag}(q_{i,j}){\trA_{-i}}^T \trA_i$ which again has spectral norm bounded by $O(k^2/mn)$.
The final term is equal to 
\begin{align*}
\E\left[\tilA_R\tilA_R^T \trA_R {\trA_R}^T\tilA_i \mathbf{1}_{\mathcal{F}_i}\right] & = \sum_{j_1,j_2\ne i} \E[(\tilA_{j_1}\tilA_{j_1}^T)(\trA_{j_2}{\trA_{j_2}}^T)\tilA_i \mathbf{1}_{\mathcal{F}_i} \mathbf{1}_{\mathcal{F}_{j_1}} \mathbf{1}_{\mathcal{F}_{j_2}}]\\
& = \sum_{j_1\ne i} \left(\sum_{j_2\ne i} q_{i,j_1,j_2} \langle \trA_{j_2},\tilA_i \rangle\langle \trA_{j_2},\tilA_{j_1} \rangle\right) \tilA_{j_1} \\
& = \tilA_{-i} v.
\end{align*}
where $v$ is a vector whose $j_2$-th component is equal to $\sum_{j_2\ne i} q_{i,j_1,j_2} \langle \trA_{j_2},\tilA_i \rangle\langle \trA_{j_2},\tilA_{j_1} \rangle$. The absolute value of $v_{j_2}$ is bounded by 
\begin{align*}
|v_{j_2}| & \le O(k^2/m^2) |\langle \trA_{j_2},\tilA_i \rangle| + O(k^3/m^3) (\sum_{j_2\ne j_1,i} (\langle \trA_{j_2},\tilA_i \rangle^2 + \langle \trA_{j_2},\tilA_{j_1} \rangle^2))\\
& \le O(k^2/m^2) |\langle \trA_{j_2},\tilA_i \rangle| + O(k^3/m^3)\|\trA\|^2 = O(k^2/m^2)(|\langle \trA_{j_2},\tilA_i \rangle|+k/n).
\end{align*}
The first inequality uses bounds for $q$'s and the AM-GM inequality, the second inequality uses the spectral norm of $\trA$. We can now bound the norm of $v$ as follows $$\|v\| \le O(k^2/m^2 \cdot \sqrt{m/n})$$ and this implies that the last term satisfies $\|\tilA_{-i}\|\|v\| \le O(k^2/mn)$. Combining all these bounds completes the proof of the lemma.
\end{proof}

We are now ready to prove that the update rule satisfies Definition~\ref{eqn:con}. This again uses Lemma~\ref{lem:closetocorrelated}, % The proof of this lemma is just a calculation and is in fact an identical calculation to the one given in the proof of Lemma~\ref{lem:checking_condtion1}, 
except that we invoke Lemma~\ref{lem:OFupdate} instead. Combining these lemmas we obtain:

\begin{lemma}\label{lem:OFtiger}
Suppose that $\tilA^s$ is $(2\delta,5)$-\near to $\trA$. Then for each $i$, $g^s_i$ as defined in Algorithm~\ref{eqn:ofrule} is $(\alpha,\beta,\epsilon)$-correlated with $\trA_i$, where $\alpha = \Omega(k/m)$, $\beta \ge \Omega(m/k)$ and $\epsilon = O(k^3/mn^2)$.
\end{lemma}

%\Tnote{infinite number of samples}

Notice that in the third step in Algorithm~\ref{eqn:ofrule} we project back into a convex set $\mathcal{B}$ which we define below. Without this modification, it seems that the update rule given in Algorithm~\ref{eqn:ofrule} does not necessarily preserve nearness. 

\begin{definition}\label{def:whiten}
Let $\mathcal{B} = \{A | A \mbox{ is } \delta_0 \mbox{ close to } A^0 \mbox{ and } \|A\| \leq 2 \|\trA \|\}$
\end{definition}

\noindent The crucial properties of this set are summarized in the following claim:

\begin{claim}
$(a)$ $\trA \in \mathcal{B}$ and $(b)$ for each $A \in \mathcal{B}$, $A$ is $(2\delta_0, 5)$-near to $\trA$
\end{claim}

\begin{proof}
The first part of the claim follows because by assumption $\trA$ is $\delta_0$-close to $A^0$ and $\|\trA - A^0\| \leq 2 \|\trA\|$. Also the second part follows because $\|A - \trA\| \leq \|A - A^0\| + \|A^0 - \trA\| \leq 4\|\trA\|$. This completes the proof of the claim.
\end{proof}

We now have the tools to analyze Algorithm~\ref{eqn:ofrule} by fitting it into the framework of Corollary~\ref{cor:tiger-convexity}. In particular, we prove that it converges to a globally optimal solution by connecting it to an approximate form of {\em projected} gradient descent:


\begin{proof} [Proof of Theorem~\ref{thm:OFupdate}]
We note that projecting into $\mathcal{B}$ ensures that at the start of each step $\|\tilA^s - \trA\| \leq 5 \|\trA\|$. Hence   $g^s_i$ is $(\Omega(k/m), \Omega(m/k), O(k^3/mn^2))$-correlated with $\trA_i$ for each $i$, which follows from  Lemma~\ref{lem:OFtiger}. Finally we can apply Corollary~\ref{cor:tiger-convexity} to complete the proof of the theorem. 
\end{proof}

%Hence by Theorem~\ref{thm:tiger-convergence} after $O(m\log n/k\eta) = O^*(\log n)$ steps the $\tilA$ matrix satisfy $\|\tilA - A\|_F \le O(\sqrt{m/n})$. In particular, since the Frobenius norm of $\tilA-A$ is not going to be larger than $O(\sqrt{m/n})$ in future iterations, the constraint set $\mathcal{B}$ will not have any effect in later iterations.

%Now we can apply Theorem~\ref{thm:tiger-convergence} on each column, and conclude that each column converges after another $O(m\log n/k\eta) = O^*(\log n)$ number of iterations.






\subsection{Removing the Systemic Error}

In this subsection, we design and analyze a new update rule whose systemic error is $n^{-\omega(1)}$. The basic idea is to choose a new decoding matrix that projects out the components along the column currently being updated. This has the effect of replacing a certain error timer in Lemma~\ref{lem:OF-simplified-update} with another term that goes to zero as $\tilA$ gets closer to $\trA$ (the earlier rules we have analyzed do not have this property). 
In particular, let $$B^{(s,i)}_i = \tilA_i \mbox{ and } B^{(s,i)}_j = \mbox{Proj}_{\tilA_i^\perp}\tilA_j$$ for $j\ne i$. We will use this as the decoding matrix when we are updating the $i$th column. Note that $B^{(s,i)}_{-i}$ (i.e. $B^{(s, i)}$ with the $i$th column removed) is now orthogonal to $\tilA_i$. We will rely on this fact when we bound the systemic error. 

\begin{algorithm}\caption{Unbiased Update Rule}\label{eqn:nonoiserule}
\vspace{0.1in}
\textbf{Initialize} $\tilA^0$ that is $(\delta_0, 2)$-near to $\trA$

\textbf{Repeat} for $s = 0, 1, ..., T$
\vspace{-0.1in}
\begin{align*}
\textbf{\textbf{Decode: }}  &  x = \textrm{threshold}_{C/2}((\tilA^s)^Ty)  \textrm{ for each sample $y$}\nonumber\\
& \bar{x}^i = \textrm{threshold}_{C/2}((B^{(s,i)})^Ty)  \textrm{ for each sample $y$, and each $i\in [m]$}\nonumber\\
\textbf{\textbf{Update: }} &  \tilA^{s+1}_i = \tilA^s_i - \eta g^{s}_i \mbox{ where } g^{s}_i =  \Exp[ (y - {B^{(s,i)}}\bar{x}^i) \sgn(\tilx)_i^T ] \textrm{ for each $i\in [m]$}\nonumber
%\tilA^{s+1}_j = \tilA^s_j - \eta g^{s}_j \mbox{ where } g^{s}_j =  \sum_{i =1}^p (y - {B^{(s,j)}}\tilx^{(i)}) \sgn(\tilx^{(i)})_j^T \nonumber
\end{align*}
\end{algorithm}

Our main theorem in this subsection is:

\begin{theorem}\label{thm:nonoiserule}
Suppose that $\tilA^0$ is $(2\delta,2)$-\near to $\trA$ and that
$\eta = \Theta(m/k)$. Then in Algorithm~\ref{eqn:nonoiserule} at each step $s$, we have
%uses $p = \widetilde{\Omega}(mk)$ fresh samples, we have
%Then if each update step in Algorithm~\ref{eqn:nonoiserule} uses $p = \widetilde{\Omega}(mk)$ fresh samples, we have
$$\|\tilA_i^s - \trA_i\|^2 \le (1-\tau)^s \|\tilA^0_i - \trA_i\|^2 + n^{-\omega(1)}$$
for some $0 < \tau < 1/2$ and for any $s=1,2, ... , T$. In particular it converges to $\trA$ geometrically with systemic error $n^{-\omega(1)}$. 
\end{theorem}


%where $\tilA^{(i)}$ is a slight twist of $\tilA$ that depends on the index $i$: 
%
%$$\tilA^{(i)}_i = \trA_i,  \quad \textrm{ and for $j\neq i$ }, \tilA^{(i)}_j  =  \Pi_{\tilA_i^{\bot}} \tilA_j = \tilA_j - \inner{\tilA_j,\tilA_i}\tilA_i/\|\tilA_i\|^2$$

%\noindent It turns out that given suitable starting conditions, this event happens with arbitrarily high probability and we will use this fact crucially in our analysis. 
%Throughout this section, we will use $\gamma$ to denote a vector whose norm can be taken to be any inverse polynomial. 


%\subsubsection{Functional Form of Update}

\noindent The proof of Theorem~\ref{thm:nonoiserule} is parallel to that of Theorem~\ref{thm:simplesample} and Theorem~\ref{thm:OFupdate}. As usual, our first step is to show that $g_s$ is correlated with $\trA$:

%Using similar analysis as Lemma~\ref{lem:OF-simplified-update}, we can show this update rule is correlated with $\trA$ with negligible error:

\begin{lemma}\label{lem:OFupdate-noerror}
Suppose that $\tilA^s$ is $(\delta,5)$-\near to $\trA$. Then for each $i$, $g^s_i$ as defined in Algorithm~\ref{eqn:nonoiserule} is $(\alpha,\beta,\epsilon)$-correlated with $\trA_i$, where $\alpha = \Omega(k/m)$, $\beta \ge \Omega(m/k)$ and $\epsilon \le n^{-\omega(1)}$.
\end{lemma}

\begin{proof} 
We chose to write the proof of Lemma~\ref{lem:OF-simplified-update} so that we can reuse the calculation here. In particular, instead of substituting $B$ for $\tilA^s$ in the calculation we can substitute $B^{(s,i)}$ instead and we get:
$$
g^{(s,i)} = p_iq_i (\lambda_i^s \tilA^s_i - \trA_i + B^{(s,i)}_{-i}\mbox{diag}(q_{i,j})B^{(s,i)T}_{-i} \trA_i) + \gamma.
$$
Recall that $\lambda^s_i = \langle \tilA_i^s, \trA_i\rangle $. Now we can write $g^{(s,i)} = p_iq_i (\tilA^s_i - \trA_i) + v$, where $$v = p_iq_i(\lambda_i^s -1)\tilA^s_i + p_iq_i B^{(s,i)}_{-i}\mbox{diag}(q_{i,j})B^{(s,i)T}_{-i} \trA_i + \gamma$$ Indeed the norm of the first term $ p_iq_i(\lambda_i^s -1)\tilA^s_i$ is smaller than $p_iq_i\|\tilA^s_i - \trA_i\|$.

Recall that the second term was the main contribution to the systemic error, when we analyzed earlier update rules. However in this case we can use the fact that $B^{(s,i)T}_{-i}\tilA^s_i = 0$ to rewrite the second term above as $$p_iq_i B^{(s,i)}_{-i}\mbox{diag}(q_{i,j})B^{(s,i)T}_{-i} (\trA_i-\tilA^s_i)$$
Hence we can bound the norm of the second term by $O(k^2/mn)\|\trA_i-\tilA^s_i\|$, which is also much smaller than $p_iq_i\|\tilA^s_i - \trA_i\|$. 

Combining these two bounds we have that $\|v\| \le p_iq_i\|\tilA^s_i - \trA_i\|/4 + \gamma$, so we can take $\zeta = \gamma = n^{-\omega(1)}$ in Lemma~\ref{lem:closetocorrelated}. We can complete the proof by invoking Lemma~\ref{lem:closetocorrelated} which implies that the $g^{(s, i)}$ is $(\Omega(k/m),\Omega(m/k), n^{-\omega(1)})$-correlated with $\tilA_i$.
\end{proof}

This lemma would be all we would need, if we added a third step that projects onto $\mathcal{B}$ as we did in Algorithm~\ref{eqn:ofrule}. However here we do not need to project at all, because the update rule maintains nearness and thus we can avoid this computationally intensive step. 


\begin{lemma}\label{lem:noerrornowhiten}
Suppose that $\tilA^s$ is $(\delta,2)$-\near to $\trA$. Then $\|\tilA^{s+1} - \trA\| \leq 2 \|\trA\|$ in Algorithm~\ref{eqn:nonoiserule}.
\end{lemma}

This proof of the above lemma parallels that of Lemma~\ref{lem:nowhiten}. We will focus on highlighting the differences in bounding the error term, to avoid repeating the same calculation. 

\begin{proof} [sketch]
We will use $\tilA$ to denote $\tilA^s$ and $B^{(i)}$ to denote $B^{(s,i)}$ to simplify the notation. 
Also let $\bar{A}_i$ be normalized so that $\bar{A}_i = \tilA_i/\|\tilA_i\|$ and then we can write $B^{(i)}_{-i} = (I-\bar{A}_i \bar{A}_i^T) \tilA_{-i}$. Hence the error term is given by $$(I-\bar{A}_i \bar{A}_i^T) \tilA_{-i} \mbox{diag}(q_{i,j}) \tilA_{-i}^T (I-\bar{A}_i \bar{A}_i^T) \trA_i$$ Let $C$ be a matrix whose columns are $C_i = (I-\bar{A}_i \bar{A}_i^T) \trA_i = A_i - \langle \bar{A}_i, \trA_i\rangle\bar{A}_i $. This implies that $\|C\| \le O(\sqrt{m/n})$. We can now rewrite the error term above as $$\tilA_{-i} \mbox{diag}(q_{i,j}) \tilA_{-i}^T C_i - (\bar{A}_i\bar{A}_i)^T\tilA_{-i}\mbox{diag}(q_{i,j}) \tilA_{-i}^T C_i$$

It follows from the proof of Lemma~\ref{lem:nowhiten} that the first term above has spectral norm bounded by $O(k/m \cdot \sqrt{m/n})$. This is because in Lemma~\ref{lem:nowhiten} we bounded the term $\tilA_{-i} \mbox{diag}(q_{i,j}) \tilA_{-i}^T \trA_i$ and in fact it is easily verified that all we used in that proof was the fact that $\|\trA\| = O(\sqrt{m/n})$, which also holds for $C$. 

All that remains is to bound the second term. We note that its columns are scalar multiples of $\bar{A}_i$, where the coefficient can be bounded as follows: $\|\bar{A}_i\|\|\tilA_{-i}\|^2 \|\mbox{diag}(q_{i,j})\| \|\trA_i\| \le O(k^2/mn)$. Hence we can bound the spectral norm of the second term iby $O(k^2/mn)\|\bar{A}\| = O^*(k/m\cdot \sqrt{m/n})$. We can now combine these two bounds, which together with the calculation in Lemma~\ref{lem:nowhiten} completes the proof. 
\end{proof}

These two lemmas directly imply Theorem~\ref{thm:nonoiserule}.





==> newinitincludeflat.tex <==
\section{Initialization}\label{sec:init}

There is a large gap between theory in practice in terms of how to initialize $\tilA$. The usual approach is to set $\tilA$ randomly or to populate its columns with samples $y^{(i)}$. But the challenge is that not only are there no known provable guarantees for these methods, in fact these methods can and do fail in practice. It is often necessary to run the initialization procedure many times in hopes of finding a good starting point. 

Here we will give a new method for initialization that is a twist on existing approaches, and for which we can show that it succeeds with very high probability. Our algorithm works by pairwise reweighting. Let $u = \trA\alpha$ and $v = \trA\alpha'$ be two samples from our model whose supports are $U$ and $V$ respectively. The main idea is that if we reweight fresh samples $y$ with a factor $\inner{y,u}\inner{y,v}$ and compute $$\widehat{M}_{u, v} = \frac{1}{p_2}  \sum_{i=1}^{p_2} \inner{y^{(i)},u}\inner{y^{(i)},v}y^{(i)}(y^{(i)})^T$$ then the top singular vectors will exactly correspond to columns $\trA_j$ where $j \in U \cap V$. 

Throughout this section we will assume that the algorithm is given two sets of samples of size $p_1$ and $p_2$ respectively. Let $p = p_1 + p_2$. We use the first set of samples for the pairs $u, v$ that are used in reweighting and we use the second set to compute $\widehat{M}_{u, v}$ (that is, the same set of $p_2$ samples is used for each $u, v$ throughout the execution of the algorithm). Our main theorem is:

\begin{theorem}
\label{thm:initmain}
Suppose that Algorithm~\ref{alg:init} is given $p_1 = \widetilde{\Omega}(m)$ and $p_2 = \widetilde{\Omega}(mk)$ fresh samples and moreover
\begin{itemize}

\item  $\trA$ is $\mu$-incoherent with $\mu= O^*(\frac{\sqrt{n}}{k \log^3 n})$

\item $m = O(n)$ and

\item $\|\trA\| \leq O(\sqrt{\frac{m}{n}})$

\end{itemize}
Then with high probability $\tilA$ is $(\delta, 2)$-near to $\trA$ where $\delta = O^*(1/\log n)$. 
\end{theorem}

\begin{algorithm}\caption{Pairwise Initialization}\label{alg:init}
\vspace{0.1in}

\textbf{Set} $L = \emptyset$

\textbf{While} $|L| < m$ choose samples $u$ and $v$

\vspace{0.1in}

$\qquad$ Set $\widehat{M}_{u, v} = \frac{1}{p_2}  \sum_{i=1}^{p_2} \inner{y^{(i)},u}\inner{y^{(i)},v}y^{(i)}(y^{(i)})^T$

\vspace{0.1in}

$\qquad$ Compute the top two singular values $\sigma_1,\sigma_2$ and top singular vector $z$ of $\widehat{M}_{u,v}$

\vspace{0.1in}

$\qquad$ \textbf{If} $\sigma_1 \ge \Omega(k/m)$ and $\sigma_2 < O^*(k/m\log m)$ 

\vspace{0.1in}

$\qquad$ $\qquad$ \textbf{If} $z$ is not within distance $1/\log m$ of any vector in $L$ (even after sign flip),  add $z$ to $L$

\vspace{0.1in}

\textbf{Set} $\widetilde{\tilA}$ such that its columns are $z \in L$ and $\tilA = \mbox{Proj}_{\mathcal{B}} \widetilde{\tilA}$ (where $\mathcal{B}$ is defined in Definition~\ref{def:whiten})

\vspace{0.1in}

\end{algorithm}



Recall that $q_{i,j} = \Pr[\trx_i\trx_j\ne 0]$. The key lemma is given below, and we defer its proof until later in the section:

\begin{lemma}\label{lem:initform}
Suppose $u = \trA\alpha$ and $v = \trA\alpha'$ are two random samples with supports $U$, $V$ respectively. Let $\beta = {\trA}^T u$ and $\beta' = {\trA}^T v$. Let $y = \trA\trx$ be random sample that is independent of $u$,$v$, then 
\begin{equation}
M_{u,v} := \E[\inner{u,y}\inner{v,y} yy^T] = \sum_{i\in U\cap V} q_ic_i\beta_i\beta'_i\trA_i{\trA_i}^T + E_1+E_2+E_3,\label{eq:initform}
\end{equation} where $q_i = \Pr[i\in S]$, $c_i = \E[{\trx_i}^4|i\ne S]$, and the error terms are:
\[
\begin{array}{rll}
E_1 & = & \sum_{i\not\in U\cap V} q_ic_i\beta_i\beta'_i \trA_i{\trA_i}^T\\
E_2 & = & \sum_{i,j\in[m],i\ne j} q_{i,j}\beta_i\beta_i' \trA_j{\trA_j}^T\\
E_3 & = & \sum_{i,j\in[m],i\ne j} q_{i,j}(\beta_i\trA_i \beta'_j{\trA_j}^T+\beta'_i\trA_i\beta_j {\trA_j}^T).
\end{array}
\]
Moreover the error terms $E_1+E_2+E_3$ has spectral norm bounded by $O^*(k/m\log n)$, $|\beta_i|\ge \Omega(1)$ for all $i\in \mbox{{\em supp}}(\alpha)$ and $|\beta'_i|\ge \Omega(1)$ for all $i\in \mbox{{\em supp}}(\alpha')$.
\end{lemma}

\noindent We will invoke this lemma several times in order to analyze Algorithm~\ref{alg:init}. 


When $u$ and $v$ share a unique dictionary element, there is only one large term in $M_{u,v}$ and the error terms are small. Hence the top singular vector of $M_{u,v}$ must be close to the corresponding dictionary element $A_i$.

\begin{lemma}
\label{lem:init}
Under the assumptions of Theorem~\ref{thm:initmain},
suppose $u = \trA\alpha$ and $v = \trA\alpha'$ are two random samples with supports $U$, $V$ respectively. When $U\cap V = \{i\}$ the top singular vector of $M_{u,v}$ is $O^*(1/\log n)$-close to $\trA_i$.
\end{lemma}

%Finally, Lemma~\ref{lem:init} follows from Wedin's Theorem:
\begin{proof} %[Proof of Lemma~\ref{lem:init}]
When $u$ and $v$ share a unique dictionary element $i$, the contribution of the first term in (\ref{eq:initform}) is just $q_ic_i\beta_i\beta'_i \trA_i{\trA_i}^T$. Moreover the coefficient $q_ic_i\beta_i\beta'_i$ is at least $\Omega(k/m)$ which follows from Lemma~\ref{lem:initform} and from the assumptions that $c_i\ge 1$ and $q_i =\Omega(k/m)$. 

On the other hand, the error terms are bounded by $\|E_1+E_2+E_3\|\le O^*(k/m\log m)$ which again by Lemma~\ref{lem:initform}. We can now apply Wedin's Theorem (see e.g. \cite{HJ}) to $$M_{u,v} = q_ic_i\beta_i\beta'_i\trA_i{\trA_i}^T + \underbrace{(E_1+E_2+E_3)}_{\mbox{perturbation}}$$ and conclude that its top singular vector must be $O^*(k/m\log m)/\Omega(k/m) = O^*(1/\log m)$-close to $\trA_i$, and this completes the proof of the lemma. 
\end{proof}

Using (\ref{eq:initform}) again, we can verify whether or not the supports of $u$ and $v$  share a unique element.

\begin{lemma}
\label{lem:initverify}
Suppose $u = \trA\alpha$ and $v = \trA\alpha'$ are two random samples with supports $U$, $V$ respectively. Under the assumption of Theorem~\ref{thm:initmain}, if the top singular value of $M_{u,v}$ is at least $\Omega(k/m)$ and the second largest singular value is at most $O^*(k/m\log m)$, then with high probability $u$ and $v$ share a unique dictionary element.
\end{lemma}

\begin{proof}
By Lemma~\ref{lem:initform} we know with high probability the error terms have spectral norm $O^*(k/m\log m)$. Here we show when that happens, and the top singular value is at least $\Omega(k/m)$, second largest singular value is at most $O^*(k/m\log m)$, then $u$ and $v$ must share a unique dictionary element.

If $u$ and $v$ share no dictionary element, then the main part in Equation (\ref{eq:initform}) is empty, and the error term has spectral norm $O^*(k/m\log m)$. In this case the top singular value of $M_{u,v}$ cannot be as large as $\Omega(k/m)$.

If $u$ and $v$ share more than one dictionary element, there are more than one terms in the main part of (\ref{eq:initform}). Let $S = U\cap V$, we know $M_{u,v} = \trA_S D_S {\trA_S}^T+E_1+E_2+E_3$ where $D_S$ is a diagonal matrix whose entries are equal to $q_ic_i\beta_i\beta'_i$. All diagonal entries in $D_S$ have magnitude at least $\Omega(k/m)$. By incoherence we know $\trA_S$ have smallest singular value at least $1/2$, therefore the second largest singular value of $\trA_SD_S{\trA_S}^T$ is at least:
$$
\sigma_2(\trA_SD_S{\trA_S}^T) \ge \sigma_{min}(\trA_S)^2\sigma_2(D_S) \ge \Omega(k/m).
$$
Finally by Weyl's theorem (see e.g. \cite{HJ}) we know $\sigma_2(M_{u,v}) \ge \sigma_2(\trA_SD_S{\trA_S}^T) - \|E_1+E_2+E_3\| \ge \Omega(k/m)$. Therefore in this case the second largest singular value cannot be as small as $O^*(k/m\log m)$.

Combining the above two cases, we know when the top two singular values satisfy the conditions in the lemma, and the error terms are small, $u$ and $v$ share a unique dictionary element.
\end{proof}

Finally, we are ready to prove Theorem~\ref{thm:initmain}. The idea is every vector added to the list $L$ will be close to one of the dictionary elements (by Lemma~\ref{lem:initverify}), and for every dictionary element the list $L$ contains at least one close vector because we have enough random samples.

\begin{proof}[Proof of Theorem~\ref{thm:initmain}]
By Lemma~\ref{lem:initverify} we know every vector added into $L$ must be close to one of the dictionary elements.
On the other hand, for any dictionary element $\trA_i$, by the bounded moment condition of $\mathcal{D}$ we know 
\[
\begin{array}{rl}
\Pr[|U\cap V| = \{i\}] & = \Pr[i\in U]\Pr[i\in V] \Pr[(U\cap V)\backslash\{i\} =\emptyset|i\in U, j\in U] \\
&\ge \Pr[i\in U]\Pr[i\in V](1 - \sum_{j\ne i, j\in [m]} \Pr[j\in U\cap V|i\in U,j\in V])\\
& = \Omega(k^2/m^2)\cdot (1-m\cdot O(k^2/m^2)) \\&= \Omega(k^2/m^2).
\end{array}
\]
Here the inequality uses union bound. Therefore given $O(m^2\log^2 n/k^2)$ trials, with high probability there is a pair of $u$,$v$ that intersect uniquely at $i$ for all $i\in [m]$. By Lemma~\ref{lem:init} this implies there must be at least one vector that is close to $\trA_i$ for all dictionary elements.

Finally, since all the dictionary elements have distance at least $1/2$ (by incoherence), the connected components in $L$ correctly identifies different dictionary elements. The output $\tilA$ must be $O^*(1/\log m)$ close to $\trA$.
\end{proof}

We now come to the proof of the main lemma:

\begin{proof}[Proof of Lemma~\ref{lem:initform}]
We will prove this lemma in three parts. First we compute the expectation and show it has the desired form. Recall that $y = \trA\trx$, and so:
\begin{eqnarray*}
M_{u,v} &=& \E_{S} \Big [\E_{\trx_S}[\inner{u, \trA_S \trx_S}\inner{v, \trA_S \trx_S}\trA_S\trx_S{\trx_S}^T{\trA_S}^T|S]\Big ]\\
&=& \E_{S} \Big [\E_{\trx_S}[\inner{\beta,\trx_S}\inner{\beta',\trx_S}\trA_S\trx_S{\trx_S}^T{\trA_S}^T|S]\Big ] \\
&=& \E_{S} \Big [ \sum_{i\in S} c_i\beta_i\beta'_i \trA_i {\trA_i}^T + \sum_{i,j\in S, i\ne j}\Big (\beta_i\beta_i' \trA_j{\trA_j}^T+\beta_i \beta'_j \trA_i {\trA_j}^T+\beta'_i \beta_j\trA_i {\trA_j}^T \Big ) \Big ] \\
&=& \sum_{i\in [m]}q_ic_i\beta_i\beta'_i \trA_i {\trA_i}^T + \sum_{i,j\in [m], i\ne j}q_{i,j}\Big (\beta_i\beta_i' \trA_j{\trA_j}^T+\beta_i \beta'_j \trA_i {\trA_j}^T+\beta'_i \beta_j \trA_i {\trA_j}^T \Big )
\end{eqnarray*}
where the second-to-last line follows because  the entries in $\trx_S$ are independent and have mean zero, and the only non-zero terms come from ${\trx_i}^4$ (whose expectation is $c_i$) and ${\trx_i}^2{\trx_j}^2$ (whose expectation is one). Equation (\ref{eq:initform}) now follows by rearranging the terms in the last line. What remains is to bound the spectral norm of $E_1, E_2$ and $E_3$. 

\vspace{0.5pc}


Next we establish some useful properties of $\beta$ and $\beta'$:

\begin{claim}
\label{claim:betabound}
With high probability it holds that $(a)$ for each $i$ we have $|\beta_i - \alpha_i| \le \frac{\mu k \log m} {\sqrt{n}}$ and $(b)$ $\|\beta\| \le O(\sqrt{mk/n})$.
\end{claim}

\noindent In particular since the difference between $\beta_i$ an $\alpha_i$ is $o(1)$ for our setting of parameters, we conclude that if $\alpha_i \neq 0$ then $C-o(1) \le |\beta_i| \le O(\log m)$  and if $\alpha_i = 0$ then $|\beta_i| \le \frac{\mu k \log m}{\sqrt{n}}$. 

\begin{proof}
Recall that $U$ is the support of $\alpha$ and let $R = U\backslash\{i\}$. Then:
$$\beta_i -\alpha_i  =  {\trA_i}^T \trA_U \alpha_U - \alpha_i =  {\trA_i}^T \trA_R \alpha_R$$
and since $\trA$ is incoherent we have that $\|{\trA_i}^T\trA_R\| \le \mu\sqrt{k/n}$. Moreover the entries in $\alpha_R$ are independent and subgaussian random variables, and so with high probability $|\inner{{\trA_i}^T \trA_R, \alpha_R}| \le \frac{\mu k \log m}{\sqrt{n}}$ and this implies the first part of the claim. 

For the second part, we can bound $\|\beta\| \leq \|\trA\|\|\trA_U\|\|\alpha\|$.  Since $\alpha$ is a $k$-sparse vector with independent and subgaussian entries, with high probability $\|\alpha\| \le O(\sqrt{k})$ in which case it follows that $\|\beta\| \le O(\sqrt{mk/n})$.
\end{proof}

%{\sc Rong: Here we proved something stronger than we need. This would imply that the algorithm works even when $m$ is a bigger polynomial of $n$ (with some extra works in the claim below). Shall we do that?}

Now we are ready to bound the error terms.

\begin{claim}
\label{claim:errorterms}
With high probability each of the error terms $E_1, E_2$ and $E_3$ in (\ref{eq:initform}) has spectral norm bounded at most $O^*(k/m\log m)$.
\end{claim}

\begin{proof}
Let $S = [m]\backslash (U\cap V)$, then $E_1 = \trA_S D_1 {\trA_S}^T$ where $D_1$ is a diagonal matrix whose entries are $q_ic_i\beta_i\beta'_i$. We first bound $\|D_1\|$. To this end, we can invoke the first part of Claim~\ref{claim:betabound} to conclude that $|\beta_i\beta'_i| \le \frac{\mu^2 k^2 \log^2 m}{n}$. Also  $q_ic_i = \Theta(k/m)$ and so $$\|D_1\| \le O\left(\frac{\mu^2 k^3\log^2 m}{m n}\right) = O\left(\frac{\mu k^2\log^2 n}{m\sqrt{n}}\right) = O^*(k/m\log m)$$ Finally $\|A_S\| \leq \|A\| \leq O(1)$ (where we have used the assumption that $m = O(n)$), and this yields the desired bound on $\|E_1\|$. 

The second term $E_2$ is a sum of positive semidefinite matrices and we will make crucial use of this fact below:
$$E_2 = \sum_{i\ne j} q_{i,j}\beta_i\beta_i' \trA_j{\trA_j}^T \preceq O(k^2/m^2) \Big (\sum_{i} \beta_i\beta_i' \Big) \Big(\sum_{j} \trA_j{\trA_j}^T\Big)  \preceq O(k^2/m^2) \|\beta\|\|\beta'\| \trA{\trA}^T.$$
Here the first inequality follows by using bounds on $q_{i,j}$ and then completing the square.  The second inequality uses Cauchy-Schwartz. We can now  invoke the second part of Claim~\ref{claim:betabound} and conclude that $\|E_2\| \le O(k^2/m^2)\|\beta\|\|\beta'\| \|\trA\|^2 \le O^*(k/m\log m)$ (where we have used the assumption that $m = O(n)$). 

For the third error term $E_3$, by symmetry we need only consider terms of the form $q_{i,j}\beta_i \beta_j' \trA_i{\trA_j}^T$. We can collect these terms and write them as $\trA Q{\trA}^T$, where $Q_{i,j} = 0$ if $i=j$ and $Q_{i,j} = q_{i,j}\beta_i\beta_j'$ if $i\ne j$. First, we bound the Frobenius norm of $Q$:
$$
\|Q\|_F = \sqrt{\sum_{i\ne j,i,j\in [m]}q_{i,j}^2\beta_i^2(\beta'_j)^2} \le \sqrt{O(k^4/m^4)(\sum_{i\in [m]}\beta_i^2)(\sum_{j\in[m]}(\beta'_j)^2)} \le O(k^2/m^2)\|\beta\|\|\beta'\|.
$$
Finally $\|E_3\| \le 2\|\trA\|^2\|Q\| \le O(m/n \cdot k^2/m^2)\|\beta\|\|\beta'\| \le O^*(k/m\log m)$, and this completes the proof of the claim. 
\end{proof}

The proof of the main lemma is now complete.
\end{proof}

\section{Sample Complexity}\label{sec:sample_complexity}

In the previous sections, we analyzed various update rules assuming that the algorithm was given the exact expectation of some matrix-valued random variable. Here we show that these algorithms can just as well use approximations to the expectation (computed by taking a small number of samples). We will focus on analyzing the sample complexity of Algorithm~\ref{eqn:simplestupdate}, but a similar analysis extends to the other update rules as well. 

\subsection{Generalizing the $(\alpha,\beta,\epsilon)$-correlated Property}

We first give a generalization of the framework we presented in Section~\ref{sec:framework}. 

\begin{definition}\label{eqn:whptiger}
A random vector $g^s$ is {\em $(\alpha, \beta,\epsilon_s)$-correlated-whp} with a desired solution $z^*$ if with probability at least $1-n^{-\omega(1)}$,
$$ \langle g^s, z^s-z^*\rangle \ge \alpha \|z^s-z^*\|^2 + \beta \|g^s\|^2 - \epsilon_s.$$
\end{definition}

This is a strong condition as it requires the random vector is well-correlated with the desired solution with very high probability. In some cases we can further relax the definition as the following:

\begin{definition}\label{eqn:randomtiger}
A random vector $g^s$ is {\em $(\alpha, \beta,\epsilon_s)$-correlated-in-expectation} with a desired solution $z^*$ if
$$ \E[\langle g^s, z^s-z^*\rangle] \ge \alpha \|z^s-z^*\|^2 + \beta\E[\|g^s\|^2] - \epsilon_s.$$
\end{definition}

We remark that $\E[\|g^s\|^2]$ can be much larger than $\|\E[g^s]\|^2$, and so the above notion is still stronger than requiring (say) that the expected vector $\E[g^s]$ is $(\alpha, \beta,\epsilon_s)$-correlated with $z^*$. 

\begin{theorem}\label{thm:random-tiger-convergence}
Suppose random vector $g^s$ is $(\alpha,\beta,\epsilon_s)$-correlated-whp with $z^*$ for $s = 1,2,\dots,T$ where $T \le \poly(n)$, and $\eta$ satisfies  $0< \eta \le 2\beta$, then  for any $s = 1,\dots,T$, 
$$ \E[\| z^{s+1}-z^*\|^2] \leq (1-2\alpha\eta) \|z^s-z^*\|^2 + 2\eta \epsilon_s$$
In particular, if $\|z^0-z^*\| \le \delta_0$ and $\epsilon_s \le \alpha \cdot o((1-2\alpha\eta)^s)\delta_0^2 + \epsilon$, 
 then the updates converge to $z^*$ geometrically with systematic error $\epsilon/\alpha$ in the sense that 
%$$\|z^s-z^*\|^2 \le (1-2\alpha\eta)^s \|z^0-z^*\| + \epsilon/\alpha.$$
$$\E[\|z^s-z^*\|^2] \le (1-2\alpha\eta)^s \delta_0^2 + \epsilon/\alpha.$$
%If $g^s$ is in addition $(\alpha,\beta,\epsilon_s)$-correlated-whp, then we know for $s \le \poly(n)$, with high probability
%$$\|z^s-z^*\|^2 \le (1-2\alpha\eta)^s \|z^0-z^*\|^2 + \epsilon/\alpha.$$
%$$\|x_s-x^*\|^2 \le (1-4\alpha\beta)^s \|z^0-z^*\| + \epsilon/(\alpha).$$
%Furthermore, if $\epsilon_s < \frac{\alpha}{2} \|z^s-z^*\|^2$ for $s = 1,\dots,T$, then 
%$$\E[\|z^s-z^*\|^2] \le (1-\alpha\eta)^s \|z^0-z^*\|^2.$$
%$$\|x_s-x^*\|^2 \le (1-2\alpha\beta)^s R^2$$
\end{theorem}

\noindent The proof is identical to that of Theorem~\ref{thm:tiger-convergence} except that we take the expectation of both sides.  

\subsection{Sample Complexity for Algorithm~\ref{eqn:simplestupdate}}

We are going to apply Theorem~\ref{thm:random-tiger-convergence} to bound the sample complexity for the simple update rule.


\begin{theorem}\label{thm:simplesample}
Suppose that $\tilA^0$ is $(2\delta,2)$-near to $\trA$ and that $\eta = \Theta(m/k)$. Then if each update rule step in Algorithm~\ref{eqn:simplestupdate} uses $p = \widetilde{\Omega}(mk)$ samples, we have 

$$\Exp[\|\tilA_i^s -\trA_i\|^2] \le (1-\tau)^s \delta_0 + O(k^2/n^2)$$

for some $0 < \tau < 1/2$ and for any $ = 1,2,...,T$, where the expectation is over the randomness of the samples.  In particular, after $s= O(\log n)$ steps, $\tilA^s$ is $O(k/n)$-close to $\trA$.  %it converges to $\trA$ geometrically with (squared) systemic error $O(k^2/n^2)$.
%Suppose the algorithm gets a initial matrix $\tilA^0$ that is $(O^*(1/\log n), 2)$-\near to $\trA$. For the simple update rule Equation~\ref{eqn:simplestupdate}, choose the step size $\eta = \Theta(m/k)$, and each step uses $\widetilde{\Omega}(mk)$ fresh samples, then in $s = O(\log n)$ steps with high probability the matrix $\tilA^s$ is $O(\sqrt{k/n})$ close to $\trA$.
\end{theorem}
%
%\begin{theorem}\label{thm:simplesample}
%Suppose the algorithm gets a initial matrix $\tilA^0$ that is $(O^*(1/\log n), 2)$-\near to $\trA$. For the simple update rule Equation~\ref{eqn:simplestupdate}, choose the step size $\eta = \Theta(m/k)$, and each step uses $\widetilde{\Omega}(mk)$ fresh samples, then in $s = O(\log n)$ steps with high probability the matrix $\tilA^s$ is $O(\sqrt{k/n})$ close to $\trA$.
%\end{theorem}

In order to prove Theorem~\ref{thm:simplesample}, we proceed in two steps. First we show when $\tilA^s$ is $(\delta_s, 2)$-\near to $\trA$, the approximate gradient is $(\alpha,\beta,\epsilon_s)$-correlated-whp with optimal solution $\trA$, with $\epsilon_s \le O(k^3/mn^2)+\alpha \cdot o(\delta_s^2)$. This allows us to use Theorem~\ref{thm:random-tiger-convergence} as long as we can guarantee the spectral norm of $\tilA^s-\trA$ is small. Next we show a version of Lemma~\ref{lem:nowhiten} which works even with the random approximate gradient, hence the nearness property is preserved during the iterations. These two steps are formalized in the following two lemmas, and we defer the proof until the end of the section.

%\begin{corollary}\label{cor:one-step}
%If $\tilA^s$ is $(2\delta,2)$-\near to $\trA$ and $\eta \le \min_i (p_iq_i(1-\delta)) = O(m/k)$, then $\tilA^s$ is $(\Omega(k/m), \Omega(m/k), O(k^3/mn^2))$-correlated with $\tilA^s$, and further
%$$ \| \tilA^{s+1}_i-\tilA_i\|^2 \leq (1-2\alpha\eta) \|\tilA^s_i-\tilA_i\|^2 +O(\eta k^2/n^2)$$
%\end{corollary}


\begin{lemma}
\label{lem:stepconcentration}
Suppose $\tilA^s$ is $(2\delta,2)$-\near to $\trA$ and $\eta \le \min_i (p_iq_i(1-\delta)) = O(m/k)$, then Let $\hat{g}^s_i$ as defined in Algorithm~\ref{eqn:simplestupdate} is $(\alpha, \beta, \epsilon_s)$-correlated-whp with $\trA_i$ with $\alpha = \Omega(k/m)$, $\beta = \Omega(m/k)$ and $\epsilon_s \le \alpha \cdot  o(\delta_s^2) + O(k^3/mn^2)$.
\end{lemma}

%The reason we need to use $\delta_s$ instead of $\|\tilA^s_i-\trA_i\|$ is because different columns may converge at different speeds. 

%\begin{lemma}
%\label{lem:stepconcentration}
%Suppose $\tilA^s$ is $(\delta,2)$-\near to $\trA$ and $\eta \le \min_i (p_iq_i(1-\delta)) = O(m/k)$, then Let $g_i = \sum_{j=1}^p (y^{(j)} - \tilA^s \trxs{j}) \sgn({\trx_i}^{(j)})$, and let $w_i$ be the number of samples $y^{(j)}(j\in[p])$ that have $i\in S$. If $p = \widetilde{\Omega}(m)$ then with high probability $w_i = \widetilde{\Omega}(k)$ and $\|g_i/w_i - \E[(y - \tilA^s \wtilx|i\in S]\| \le (o(\delta_s)+O(\sqrt{k/n}))$. In particular, this implies the vector is $(\alpha, \beta, \epsilon_s)$-correlated-whp with $A_i$ with $\alpha = \Omega(k/m)$, $\beta = \Omega(m/k)$ and $\epsilon_s \le \alpha \cdot  o(\delta_s^2) + O(k^2/mn)$.
%\end{lemma}

%The proof of this lemma treats $g_i$ as sum of independent random vectors, and use vector Bernstein's inequality to give a concentration bound. 


\begin{lemma}\label{lem:nearnessconcentration}
Suppose $\tilA^s$ is $(\delta_s, 2)$-\near to $\trA$ with $\delta_s = O^*(1/\log n)$, and number of samples used in step $s$ is $p = \widetilde{\Omega}(mk)$, then with high probability $\tilA^{s+1}$ satisfies $\|\tilA^{s+1}-\trA\| \le 2\|\trA\|$.
\end{lemma}

The idea of proving these lemmas is simply bounding the difference of $\hat{g}_i^s = \frac{1}{p}\cdot\sum_{i=1}^p (y^{(i)} - \tilA^s \tilx^{(i)}) \sgn(\tilx^{(i)})^T$ with $\Exp\left[(y - \tilA^s \tilx) \sgn(\tilx)^T\right]$ by concentration inequality. 

\begin{lemma}
Suppose $\tilA^s$ is $(\delta_s, 2)$-\near to $\trA$ with $\delta_s = O^*(1/\log n)$, and number of samples used in step $s$ is $p = \widetilde{\Omega}(mk)$, then with high probability $\|\hat{g}_i^s - g_i^s\| \le o(k/m \cdot \sqrt{m/n})$. 
\end{lemma}

Based on this, for Lemma~\ref{lem:stepconcentration}, we only recall $g_i^s$ is correlated with $\trA_i$, then we have $\hat{g}_i^s$ is correlated-whp with $\trA_i$ as well. The proof of Lemma~\ref{lem:nearnessconcentration} mainly involves using matrix Bernstein's inequality to bound the fluctuation of the spectral norm of $A^{s+1}$.

Combining these Lemma~\ref{lem:stepconcentration} and Lemma~\ref{lem:nearnessconcentration}, and apply Theorem~\ref{thm:random-tiger-convergence}, we get Theorem~\ref{thm:simplesample} directly.

\subsection{Sample Complexity for Algorithm~\ref{alg:init}}

For the initialization procedure, when computing the reweighted covariance matrix $M_{u,v}$ we can only take the empirical average over samples. Here we show with only $\widetilde{\Omega}(mk)$ samples, the difference between the true $M_{u,v}$ matrix and the estimated $M_{u,v}$ matrix is already small enough.

\begin{lemma}
\label{lem:initconcentration}
In Algorithm~\ref{alg:init}, if $p = \widetilde{\Omega}(mk)$ then with high probability $\|M_{u,v} - \widehat{M}_{u,v}\| \le O^*(k/m\log n)$. 
\end{lemma}

Notice that although in the initialization procedure, we need to estimate $M_{u,v}$ for many pairs $u$ and $v$, the samples used for different pairs do not need to be independent. Therefore we can partition the data into two parts, use the first part to sample pairs $u,v$, and use the second part to estimate $M_{u,v}$. In this way the whole initialization algorithm also takes $\widetilde{\Omega}(mk)$ samples.

\subsection{Proofs of Auxiliary Lemmas}

Here we prove Lemma~\ref{lem:stepconcentration}, Lemma~\ref{lem:nearnessconcentration}, and Lemma~\ref{lem:initconcentration} which will follow from various versions of the Bernstein inequality. We first recall Bernstein's inequality that we are going to use several times in this section.  Let $Z$ be a random variable (which could be a vector or a matrix) chosen from some distribution $\mathcal{D}$ and let $Z^{(1)}, X^{(2)}, ..., Z^{(p)}$ be $p$ independent and identically distributed (i.i.d.) samples from $\mathcal{D}$.  The Bernstein inequality says that if $\|Z^{(j)}\|\le R$ almost surely and $\E[(Z^{(j)})^2] \le \sigma^2$, then 
\begin{eqnarray}
\frac{1}{p}\|\sum_{i=1}^p Z^{(i)}\| \leq \widetilde{O}\left(\frac{R}{p} + \sqrt{\frac{\sigma^2}{p}}\right) \label{eqn:bernstein}
\end{eqnarray} 

 with high probability. The proofs below will involve computing good bounds on $R$ and $\sigma^2$. However in our setting, the random variables will not be bounded almost surely. We will use the following technical lemma to handle this issue. 

\begin{lemma}\label{lem:general_bernstein}
Suppose that the distribution of $Z$ satisfies $\Pr[\|Z\| \ge R (\log (1/\rho))^C] \le 1-\rho$ for some constant $C > 0$, then 
\begin{itemize}

\item[(a)] If $p = n^{O(1)}$ then $\|Z^{(j)}\| \leq \widetilde{O}(R)$ holds for each $j$ with high probability and 

\item[(b)] $\|\E[Z \mathbf{1}_{\|Z\| \ge \widetilde{\Omega}(R)}]\| = n^{-\omega(1)}$. 
\end{itemize}
\end{lemma}

\noindent In particular, if $\frac{1}{p} \sum_{j=1}^p Z^{(j)} (1-\mathbf{1}_{\|Z^{(j)}\| \ge \widetilde{\Omega}(R)})$ is concentrated with high probability, then $\frac{1}{p}\sum_{j=1}^p Z^{(j)}$ is too.


\begin{proof}
The first part of the lemma follows from choosing $\rho = n^{-\log n}$ and applying a union bound. The second part of the lemma follows from 
\begin{align*}
\E[Z\mathbf{1}_{\|Z\| \ge R\log^{2c} n}]& \le \E[\|Z\|\mathbf{1}_{\|Z\| \ge R\log^{2c} n}]\\
& = R\log^{2c}n\Pr[\|Z\|\ge R\log^{2c}n] + \int_{R\log^{2c}n}^\infty \Pr[\|Z\|\ge t] dt = n^{-\omega(1)}.
\end{align*}
and this completes the proof. 
\end{proof}

All of the random variables we consider are themselves products of subgaussian random variables, so they satisfy the tail bounds in the above lemma. In the remaining proofs we will focus on bounding the norm of these variables with high probability.

\begin{proof}[Proof of Lemma~\ref{lem:stepconcentration}] Since $s$ is fixed throughout, we will use $\tilA$ to denote $\tilA^s$. Also we fix $i$ in this proof. Let $S$ denote the support of $\trx$. Note that $\hat{g}_i$ is a sum of random variable of the form $(y-\tilA \tilx)\sgn(\tilx_i)$. Therefore we are going to apply Bernstein inequality for proving $\hat{g}_i$ concentrates around its mean $g_i$. Since Bernstein is typically not tight for sparse random varaibles like in our case. We study the concentration of the random variable $Z := (y-\tilA \tilx)\sgn(\tilx_i)\mid i\in S$ first. We prove the following technical lemma at the end of this section.  

\begin{lemma}\label{lem:sample_conentration}
Let $Z^{(1)},\dots, Z^{(\ell)}$ be i.i.d random variables with the same distribution as $Z:= (y-\tilA \tilx)\sgn(\tilx_i)\mid i\in S$. Then when $\ell = \widetilde{\Omega}(k)$, 
$$\|\frac{1}{\ell}\sum_{j=1}^{\ell} Z^{(j)}- \Exp[Z] \|\le o(\delta_s) + O(k/n)$$ 
\end{lemma}

Let $W = \{j: i \in \supp(\trxs{j})\}$ and then we have that $\hat{g}_i= \frac{|W|}{p}\cdot \frac{1}{|W|}\sum_j (y^{(j)}-\tilA \tilx^{(j)})\sgn(\tilx^{(j)}_i)$. Note that $\frac{1}{|W|}\sum_j (y^{(j)}-\tilA \tilx^{(j)})\sgn(\tilx^{(j)}_i)$ has the same distribution as $\frac{1}{\ell}\sum_{j=1}^{\ell} Z^{(j)}$ for $\ell = |W|$, and indeed by concentration we have $\ell = |W| = \widetilde{\Omega}(k)$ when $p = \widetilde{\Omega}(mk)$. Also note that $\Exp[(y-\tilA \tilx)\sgn(\tilx_i)] = q_i\cdot \Exp[Z]$ with $q_i = O(k/m)$. Therefore by Lemma~\ref{lem:sample_conentration} we have that 

$$\|\hat{g}_i - g_i\| \le O(k/m) \| O(k/m)\cdot\|\frac{1}{\ell}\sum_{j=1}^{\ell} Z^{(j)}- \Exp[Z] \| \le O(k/m)\cdot (o(\delta_s) + O(k/n))$$ 


%We can now combine the above claims and apply the vector Bernstein inequality.  Since $p = \widetilde{\Omega}(m)$ we have that with high probability $w_i = \widetilde{\Omega}(k)$. Then $\|g_i/w_i - \E[(y - \tilA^s \wtilx|i\in S]\| \le (o(\delta_s)+O(\sqrt{k/n}))$. 
By the proof of Lemma~\ref{lem:checking_condtion1} we know $g_i= \E[(y - \tilA\wtilx)\sgn(x_i) ]$ is $(\Omega(k/m), \Omega(m/k), O(k^3/mn^2))$-correlated with $\trA$, and hence we have

\begin{align*}
\langle \hat{g}_i, \tilA_i - \trA_i\rangle & = \langle g_i,\tilA_i-\trA_i\rangle+ \langle \hat{g}_i - g_i,\tilA_i-\trA_i\rangle \\
& \ge \Omega(k/m) \|\tilA_i-\trA_i\|^2 + \Omega(m/k) \|g_i\|^2  - O(k^3/(mn^2)) - O(\delta_s\cdot k/m \cdot (\delta_s + k/n))\\
& \ge \Omega(k/m) \|\tilA_i-\trA_i\|^2 + \Omega(m/k)\|g_i\|^2  - O(\delta_s^2 + k^3/(mn^2))\\
& \ge \Omega(k/m) \|\tilA_i-\trA_i\|^2 + \Omega(m/k)\|\hat{g}_i\|^2  - O(\delta_s^2 + k^3/(mn^2))\\
\end{align*}

where the last inequality uses $\|\hat{g}_i\|^2 \le 2\|g_i\|^2+ 2\|\hat{g}_i - g_i\|^2 \le  2\|g_i\|^2 + O(\delta_s^2 + k^2/n^2)$. This completes the proof of the Lemma. 
 

$\|g_i/w_i\|^2 \le 2\|\E[(y - \tilA \wtilx)|i\in S]\|^2+ 2\|g_i/w_i -\E[(y - \tilA \wtilx)|i\in S]\|^2 \le  2\|\E[(y - \tilA \wtilx)|i\in S]\|^2 + O(\delta_s^2 + k/n)$, therefore $g_i/w_i$ is $(\Omega(1), \Omega(1), o(\delta_s)+O(k/n))$-correlated-whp with $A_i$.

%Finally, we notice that the estimated gradient $\frac{1}{p} \sum_{i=1}^p \sum_{j=1}^p (y^{(j)} - \tilA^s \trxs{j}) \sgn(\trxs{j}_i) = \Theta(k/m) \cdot g_i/w_i$, which then implies the lemma.



%The random variable we are interested in is $(y-\tilA \tilx)\sgn(\tilx_i)$ conditioned on $i\in S$, and we will give a bound on its norm that holds with high probability and bound its variance. 
\end{proof}
\begin{proof}[Proof of Lemma~\ref{lem:sample_conentration}]
We apply the Bernstein's inequality stated in equation~\ref{eqn:bernstein} with the additional technical lemma~\ref{lem:general_bernstein} in order to prove the concentration inequality we desired. We are going to control the maximum norm of $Z$ and as well as the variance of $Z$ using Claim~\ref{claim:stepinfinitynorm} and Claim~\ref{claim:var} as follows: 
\begin{claim}
\label{claim:stepinfinitynorm}
 $\|Z\| = \|(y-\tilA\tilx)\sgn(\tilx_i)\| \le \widetilde{O}(\mu k/\sqrt{n} + k \delta_s^2 + 1)$ holds with high probability
\end{claim}

\begin{proof}
We write $ y-\tilA\tilx = (\trA_S - \tilA_S \tilA_S^T \trA_S) \trx_S = (\trA_S - \tilA_S) \trx_S + \tilA_S(I - \tilA_S^T \trA_S) \trx_S$ and we will bound each term. For the first term, since $\tilA$ is $\delta_s$-close to $\trA$, we have that $\|\trA_S-\tilA_S\|_F \le \delta_s \sqrt{k}$. And for the second term, we have
\begin{align*}
\|\tilA_S(\tilA_S^T \trA_S - I)\|_F
&\le \|\tilA_S\|\|(\tilA_S^T \trA_S - I)\|_F\\
& \le (\|\trA_S\|+\delta_s \sqrt{k}) (\| (\tilA_S - \trA_S)^T \trA_S\|_F + \|{\trA_S}^T \trA_S - I\|_F)\\
& \le (2+\delta_s \sqrt{k}) (\|\trA_S\|\|\tilA_S - \trA_S\|_F + \mu k/\sqrt{n})  \le O(\mu k/\sqrt{n} + \delta_s^2 k + 1).
\end{align*}
Here we have repeatedly used the bound $\|U V\|_F \le \|U\|\|V\|_F$ and the fact that $\trA$ is $\mu$ incoherent which implies $\|\trA_S\| \le 2$. Recall that the entries in $\trx_S$ are chosen independently of $S$ and are subgaussian. Hence if $M$ is fixed then $\|M\trx_S\| \le \widetilde{O}(\|M\|_F)$ holds with high probability. And so
$$\|(y-\tilA\tilx)\sgn(\tilx_i)\| \leq \widetilde{O}(\|\trA_S-\tilA_S\|_F + \|\tilA_S(\tilA_S^T \trA_S - I)\|_F) \leq  \widetilde{O}(\mu k/\sqrt{n} + k \delta_s^2 + 1)$$ which holds with high probability and this completes the proof. 
\end{proof}

Next we bound the variance.
\begin{claim}\label{claim:var}
$\Exp[\|Z\|^2] = \E[\|(y-\tilA\tilx)\sgn(\tilx_i)\|^2|i\in S] \le O(\delta_s^2 + k^2/n^2)$.
\end{claim}

\begin{proof}
We can again use the fact that $ y-\tilA\tilx = (\trA_S - \tilA_S \tilA_S^T \trA_S) \trx_S $ and that $\trx_S$ is conditionally independent of $S$ and conclude
$$\E[\|(y-\tilA\tilx)\sgn(\tilx_i)\|^2|i\in S]  = \mbox{tr}\Big(\E_{S\ni i}[(\trA_S - \tilA_S \tilA_S^T \trA_S)(\trA_S - \tilA_S \tilA_S^T \trA_S)^T]\Big)$$
where $\mbox{tr}(\cdot)$ is the trace of a matrix and we used the fact that both the expectation and the trace are linear operators.

Let $R = S\backslash \{i\}$. We can break up the terms accordingly as we did in Lemma~\ref{lem:OFupdate}. There are terms that involve either $A_RA_R^T$ or $\tilA_R\tilA_R^T$ or both, and the remaining term is $(\trA_i - \langle \trA_i,\tilA_i\rangle \tilA_i)(\trA_i - \langle \trA_i,\tilA_i\rangle \tilA_i)^T$. In fact the contribution of all the terms of the first type can be bounded by $O(k^2/n^2)$. This follows directly from the calculation in Lemma~\ref{lem:OFupdate}), where we had to bound these same quadratic terms. The contribution of the remaining term is equal to $\|(\trA_i - \langle \trA_i,\tilA_i\rangle \tilA_i)\|^2 = O(\delta_s^2)$, and this completes the proof. 
\end{proof}

Finally we are ready to apply Lemma~\ref{lem:general_bernstein}. Set $R = \mu k/\sqrt{n} + k \delta_s^2 + 1$. Then by claim~\ref{claim:stepinfinitynorm}, claim~\ref{claim:var} and Bernstein Inequality, we know that the truncated version of $Z$ concentrates:
$$\|\frac{1}{\ell}\sum_{j=1}^{\ell} Z^{(j)}(1-\mathbf{1}_{\|Z^{(j)}\|\ge \Omega(R)})- \Exp[Z(1-\mathbf{1}_{\|Z\|\ge \Omega(R)})] \|\le o(\delta_s) + O(k/n)$$ 
Then by Lemma~\ref{lem:general_bernstein}, we have that $\sum_j Z^{(j)}$ also concentrates: 
$$\|\frac{1}{\ell}\sum_{j=1}^{\ell} Z^{(j)}- \Exp[Z] \|\le o(\delta_s) + O(k/n)$$ 
and this completes the proof.\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:nearnessconcentration}]
We will apply the matrix Bernstein inequality. In order to do this, we need to establish bounds on the spectral norm and on the variance. For the spectral norm bound, we have $\|(y - \tilA^s \wtilx) \sgn(\wtilx)^T\| = \|(y - \tilA^s \wtilx)\|\|\sgn(\wtilx)\| = \sqrt{k}\|(y - \tilA^s \wtilx)\|$. We can now use Claim~\ref{claim:stepinfinitynorm} to conclude that $\|(y - \tilA^s \wtilx)\| \le \widetilde{O}(k)$, and hence $\|(y - \tilA^s \wtilx) \sgn(\wtilx)\| \le \widetilde{O}(k^{3/2})$ holds with high probability.  

For the variance, we need to bound both $\E[(y - \tilA^s \wtilx) \sgn(\wtilx)^T\sgn(\wtilx)(y - \tilA^s \wtilx)^T]$ and $\E[\sgn(\wtilx)(y - \tilA^s \wtilx)^T(y - \tilA^s \wtilx) \sgn(\wtilx)^T]$. The first term is equal to $k\E[(y - \tilA^s \wtilx)(y - \tilA^s \wtilx)^T]$. Again, the bound follows from the calculation in Lemma~\ref{lem:OFupdate} and we conclude that $$\|\E[(y - \tilA^s \wtilx) \sgn(\wtilx)^T\sgn(\wtilx)(y - \tilA^s \wtilx)^T] \|\leq O(k^2/n)$$
To bound the second term we note that $$\E[\sgn(\wtilx)(y - \tilA^s \wtilx)^T(y - \tilA^s \wtilx) \sgn(\wtilx)^T] \preceq \widetilde{O}(k^2)\E[\sgn(\wtilx)\sgn(\wtilx)^T] \preceq \widetilde{O}(k^3/m) I$$ Moreover we can now apply the matrix Bernstein inequality and conclude that when the number of samples is at least $\widetilde{\Omega}(mk)$ we have $$\|\frac{1}{p} \sum_{j=1}^p (y^{(j)} - \tilA^s \trxs{j}) \sgn(\trxs{j})^T - \E[(y - \tilA^s \wtilx) \sgn(\wtilx)^T\| \le O^*(k/m \cdot \sqrt{m/n})$$ and this completes the proof. 
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:initconcentration}]
Again in order to apply the matrix Bernstein inequality we need to bound the spectral norm and the variance of each term of the form $\langle u,y\rangle\langle v,y\rangle yy^T$ . We make use of the following claim to bound the magnitude of the inner product:

\begin{claim}
$|\langle u,y\rangle| \le \widetilde{O}(\sqrt{k})$ and $\|y\| \le \widetilde{O}(\sqrt{k})$ hold with high probability
\end{claim}

\begin{proof}
Since $u = \trA\alpha$ and because $\alpha$ is $k$-sparse and has subgaussian non-zero entries we have that $\|u\| \le \widetilde{O}(\sqrt{k})$, and the same bound holds for $y$ too. Next we write $|\langle u,y\rangle| = |\langle {\trA}_S^Tu, \trx_S\rangle|$ where $S$ is the support of $\trx$. Moreover for any set $S$, we have that $$\|{\trA_S}^Tu\| \le \|\trA_S\|\|u\| \le \widetilde{O}(\sqrt{k})$$ holds with high probability, again because the entries of $\trx_S$ are subgaussian we conclude that $|\langle u,y\rangle|\le \widetilde{O}(\sqrt{k})$ with high probability.
\end{proof}

\noindent This implies that $\|\langle u,y\rangle\langle v,y\rangle yy^T \| \leq \widetilde{O}(k^2)$ with high probability.

Now we need to bound the variance:

\begin{claim}
$\|\E[\langle u,y\rangle^2\langle v,y\rangle^2 yy^Tyy^T]\| \le \widetilde{O}(k^3/m)$
\end{claim}

\begin{proof}
We have that with high probability $\|y\|^2 \le \widetilde{O}(k)$ and $\langle u,y\rangle^2 \le \widetilde{O}(k)$, and we can apply these bounds to obtain $$\E[\langle u,y\rangle^2\langle v,y\rangle^2 yy^Tyy^T] \preceq \widetilde{O}(k^2)\E[\langle v,y\rangle^2 yy^T]$$ On the other hand, notice that $\E[\langle v,y\rangle^2 yy^T] = M_{v,v}$ and using Lemma~\ref{lem:initform} we have that $\|\E[\langle v,y\rangle^2 yy^T]\| \le O(k/m)$. Hence we conclude that the variance term is bounded by $\widetilde{O}(k^3/m)$.
\end{proof}

Now we can apply the matrix Bernstein inequality and conclude that when the number of samples is $p = \widetilde{\Omega}(mk)$ then $$\|\hat{M}_{u,v} - M_{u,v}\| \leq \widetilde{O}(k^2)/p + \sqrt{\widetilde{O}(k^3/mp)} \le O^*(k/m\log n)$$ with high probability, and this completes the proof. 
\end{proof}

==> togetherincludeflat.tex <==
\section{Proofs of Auxiliary Lemmas}
\label{sec:hypothesis}

%The goal of this section is to prove Lemma~\ref{lem:checking_condtion0}. We show that when $\tilA$ is appropriately initialized to be  $\delta$-close to the true $\trA$, and 
%update rules ensure that the solution inductively satisfies to be $(2\delta,2)$-near to $\trA$, which then imply the statement of Lemma~\ref{lem:checking_condtion0}.

%In the first subsection we compute the expectation in Equation (\ref{eqn:simplestupdate}) and give its form. In the next part we show when the current $\tilA^s$ is $(2\delta,2)$-\near to $A$, then the update direction $g^s$ $(\alpha,\beta,\epsilon)$-points to $\trA$. Finally we show that assuming $\tilA^s$ is $(\delta,2)$-close to $\trA$, so is $\tilA^{s+1}$. Based on these, an easy induction on $s$ completes the argument. 

In Lemma~\ref{lem:OF-simplified-update} we gave a new (and more useful) expression that describes the update direction under the assumptions of our generative model. Here we will make crucial use of Lemma~\ref{lem:OF-simplified-update} in order to prove that $g^s_i$ is $(\alpha,\beta,\epsilon)$-correlated with $A_i$ (Lemma~\ref{lem:checking_condtion1}). Moreover we use Lemma~\ref{lem:OF-simplified-update} again to show that $\|\tilA^{s+1} - \trA\|\le 2\|\trA\|$ (Lemma~\ref{lem:nowhiten}). Together, these auxiliary lemmas imply that the column-wise error decreases in the next step and moreover the errors across columns are uncorrelated. 

We assume that each iteration of Algorithm~\ref{eqn:simplestupdate} takes infinite number of samples, and prove the corresponding simplified version of Theorem~\ref{thm:simplestupdate}. The proof of this Theorem highlights the essential ideas of behind the proof of the Theorem~\ref{thm:simplestupdate}, which can be found at Section~\ref{sec:sample_complexity}. 

\begin{theorem}\label{thm:simplestupdate-infinitesample}
Suppose that $\tilA^0$ is $(2\delta,2)$-\near to $\trA$ and that
$\eta = \Theta(m/k)$. Then if each update step in Algorithm~\ref{eqn:simplestupdate} uses infinite number of samples at each iteration, we have
$$\|\tilA_i^s - \trA_i\|^2\le (1-\tau)^s \|\tilA^0_i - \trA_i\|^2 + O(k^2/n^2)$$
for some $0 < \tau < 1/2$ and for any $s=1,2, ... , T$. In particular it converges to $\trA$ geometrically with systemic error $O(k^2/n^2)$. 
\end{theorem}

The proof is deferred to the end of this section. 


%{\sc Sanjeev; To be done; pls rearrange}

%In this section, we show that under some assumptions on the current guess $\tilA$, the next iteration will be closer to the true $A$. These assumptions are satisfied by our initialization procedure, and they are also satisfied after the whitening procedure.

%Throughout this section,  we assume that we obtained from initialization an estimate $\tilA^0$ of matrix $A$ with column-wise error at most $c/\log n$ for some sufficiently small constant $c$, that is, $$\|\tilA^0_i - \trA_i\| \le c/\log n, \quad\forall i\in [m]$$

%\input{functionalflat}
\subsection{Making Progress}\label{sec:progress}

In Lemma~\ref{lem:OF-simplified-update} we showed that $g^s_i = p_i q_i ( \lambda_i\tilA_i^s - \trA_i +\epsilon^s_i + \gamma)$ where $\lambda_i = \inner{\tilA_i, \trA_i}$. Here we will prove that $g_i^s$ is $(\alpha,\beta,\epsilon)$-correlated with $\trA_i$. Recall that we fixed $\delta = O^*(1/\log n)$. The main intuition is that $g^s_i$ is mostly equal to $p_iq_i (\tilA_i^s - \trA_i)$ with a small error term.


\begin{lemma}
\label{lem:checking_condtion1}
\label{lem:closetocorrelated}
If a vector $g^s_i$ is equal to $4\alpha (\tilA_i^s - \trA_i) + v$ where $\|v\| \le \alpha \|\tilA_i^s - \trA_i\| + \zeta$, then $g^s_i$ is $(\alpha, 1/100\alpha, \zeta^2/\alpha)$-correlated with $\trA_i$, more specifically,
$$
\langle g^s_i, \tilA^s_i - \trA_i\rangle \ge  \alpha \|\tilA^s_i -\trA_i \|^2 + \frac{1}{100\alpha} \|g_i\|^2 - \zeta^2/\alpha.
$$
\end{lemma}


\iffalse
\begin{lemma}\label{lem:checking_condtion1} If $\tilA^s$ is $(2\delta,2)$-\near to $\trA$, then 
$$\langle g^s_i, \tilA^s_i - \trA_i\rangle \ge  \frac{1}{p_iq_i(4+2\delta)}\|g_i\|^2 + \frac{(p_iq_i)(1-\delta)}{2}\|\tilA_i -\trA_i \|^2 - O(k^2/mn).$$
\end{lemma}
\fi

\noindent In particular,  $g_i^s$ is 
$(\alpha,\beta,\epsilon)$-correlated with $\trA_i$, where  $\alpha  = \Omega(k/m)$, $\beta \ge  \Omega(m/k)$ and $\epsilon = O(k^3/mn^2)$. We can now apply Theorem~\ref{thm:tiger-convergence} and conclude that the column-wise error gets smaller in the next step:

\begin{corollary}\label{cor:one-step}
If $\tilA^s$ is $(2\delta,2)$-\near to $\trA$ and $\eta \le \min_i (p_iq_i(1-\delta)) = O(m/k)$, then $g_i^s= p_i q_i ( \lambda_i\tilA_i^s - \trA_i +\epsilon^s_i + \gamma)$ is $(\Omega(k/m), \Omega(m/k), O(k^3/mn^2))$-correlated with $\trA_i$, and further
$$ \| \tilA^{s+1}_i-\trA_i\|^2 \leq (1-2\alpha\eta) \|\tilA^s_i-\trA_i\|^2 +O(\eta k^2/n^2)$$
\end{corollary}

\begin{proof}[Proof of Lemma~\ref{lem:checking_condtion1}]
Throughout this proof $s$ is fixed and so we will omit the superscript $s$ to simplify notations. By the assumption, $g_i$ already has a component that is pointing to the correct direction $\tilA_i-\trA_i$, we only need to show that the norm of the extra term $v$ is small enough. First we can bound the norm of $g_i$ by triangle inequality: $\|g_i\| \le \|4\alpha(\tilA_i-\trA_i)\|+\|v\| \le 5\alpha\|(\tilA_i-\trA_i)\| + \zeta$, therefore $\|g_i\|^2 \le 50\alpha^2 \|(\tilA_i-\trA_i)\|^2 + 2\zeta^2$. Also, we can bound the inner-product between $g_i$ and $\tilA_i - \trA_i$ by $\langle g_i, \tilA_i - \trA_i\rangle \ge 4\alpha \|\tilA_i - \trA_i\|^2 - \|v\|\|\tilA_i - \trA_i\|$. 

Using these bounds, we will show $\langle g_i, \tilA_i - \trA_i\rangle -  \alpha \|\tilA_i -\trA_i \|^2 - \frac{1}{100\alpha} \|g_i\|^2 + \zeta^2/\alpha \ge 0$. Indeed we have
\begin{flalign*}
& \langle g_i, \tilA_i - \trA_i\rangle -  \alpha \|\tilA_i -\trA_i \|^2 - \frac{1}{100\alpha} \|g_i\|^2 + \zeta^2/\alpha  \\ &\qquad \ge \quad 4\alpha \|\tilA_i -\trA_i \|^2 - \|v\|\|\tilA_i - \trA_i\| - \alpha \|\tilA_i -\trA_i \|^2-\frac{1}{100\alpha} \|g_i\|^2 + \zeta^2/\alpha\\
&\qquad \ge \quad  3\alpha \|\tilA_i -\trA_i \|^2 - (\alpha \|\tilA_i - \trA_i\|+\zeta)\|\tilA_i - \trA_i\|-\frac{1}{100\alpha} (50\alpha^2\|(\tilA_i-\trA_i)\|^2+2\zeta^2) + \zeta^2/\alpha \\
&\qquad \ge \quad  \alpha \|\tilA_i -\trA_i \|^2 - \zeta \|\tilA_i - \trA_i\| + \frac{1}{4} \zeta^2/\alpha \\ 
&\qquad = \quad(\sqrt{\alpha}\|\tilA_i-\trA_i\|-\zeta/2\sqrt{\alpha})^2\ge 0.
\end{flalign*}
\noindent This completes the proof of the lemma.
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:one-step}]
We use the form in Lemma~\ref{lem:OF-simplified-update}, $g^s_i = p_i q_i ( \lambda_i\tilA_i^s - \trA_i +\epsilon^s_i + \gamma)$ where $\lambda_i = \inner{\tilA_i, \trA_i}$. We can write $g^s_i = p_iq_i (\tilA_i^s-\trA_i) + p_iq_i((1-\lambda_i)\tilA_i^s + \epsilon^s_i + \gamma)$, so when applying Lemma~\ref{lem:closetocorrelated} we can use $4\alpha = p_iq_i = \Theta(k/m)$ and $v = p_iq_i((1-\lambda_i)\tilA_i^s + \epsilon^s_i + \gamma)$. The norm of $v$ can be bounded in two terms, the first term $p_iq_i(1-\lambda_i)\tilA_i^s$ has norm $p_iq_i (1-\lambda_i)$ which is smaller than $p_iq_i \|\tilA_i^s-\trA_i\|$, and the second term has norm bounded by $\zeta = O(k^2/mn)$.

By Lemma~\ref{lem:closetocorrelated} we know the vector $g^i_s$ is $(\Omega(k/m), \Omega(m/k), O(k^3/mn^2))$-correlated with $\tilA^s$. Then by Theorem~\ref{thm:tiger-convergence} we have the last part of the corollary.
\end{proof}

\iffalse
\begin{proof}[Proof of Lemma~\ref{lem:checking_condtion1}]
Throughout this proof $s$ is fixed and so we will omit the superscript $s$ for notational convenience. Moreover we define $h_i = \lambda_i\tilA_i - \trA_i +\epsilon_i + \gamma$ and $\bar{h}_i =  \lambda_i \tilA_i - \trA_i $. Then it straightforward to compute
$$\langle \bar{h}_i, \tilA_i  - \trA_i\rangle = \|\bar{h}_i\|^2 - \lambda_i (1-\lambda_i )(1-\|\tilA_i \|^2)$$ 
Note that $\tilA_i$ is not necessarily a unit vector, but is close to a unit vector since its Euclidean distance to $\trA_i$ is at most $\delta$. 
If the second term on right hand side is non-positive, then we get the lower bound $\langle \bar{h}_i, \tilA_i  - \trA_i\rangle \ge \|\bar{h}_i\|^2 $. Otherwise we bound it as follows:
\begin{align*}
\|\bar{h}_i\|^2 &= \left(\lambda_i \right)^2\left(\|\tilA_i \|^2-1\right) + 1 - \left(\lambda_i \right) ^2  \\
& \ge \left(\lambda_i \right)^2 \left(\|\tilA_i \|^2-1\right)  + 1 - \|\tilA_i \|^2 \\
& = (1+\lambda_i )(1-\lambda_i )\left(\|\tilA_i \|^2-1\right) \\
&\ge \frac{2+\delta }{1+\delta }\cdot \lambda_i (1-\lambda_i )\left(\|\tilA_i \|^2-1\right)
\end{align*}
where the equalities follow simple manipulations and the first inequality uses the fact that $\lambda_i  = \langle \tilA_i, \trA_i\rangle \le \|\tilA_i \|$. 
Therefore, we get that $\lambda_i (1-\lambda_i )(1-\|\tilA_i \|^2) \le \frac{1+\delta }{2+\delta }\|\bar{h}_i\|^2$, and it follows that 
$$\langle \bar{h}_i, \tilA_i  - \trA_i\rangle = \|\bar{h}_i\|^2 - \lambda_i (1-\lambda_i )(1-\|\tilA_i \|^2) \ge \frac{1}{2+\delta }\|h_i\|^2$$ 

Next we write $\langle \bar{h}_i, \tilA_i  - \trA_i \rangle = 
\lambda_i \|\tilA_i  - \trA_i \|^2 + (1-\lambda_i )^2\ge  \lambda_i \|\tilA_i  - \trA_i \|^2$ and combining these inequalities yields
$$\langle \bar{h}_i, \tilA_i  - \trA_i\rangle \ge \frac{1}{4+2\delta }\|\bar{h}_i\|^2 + \frac{\lambda_i }{2}\|\tilA_i  - \trA_i \|^2$$

Next we show that moving from $\bar{h}_i$ to $h_i$ does not incur much additional error. Note that $\|\trA_i\|= 1, \|\tilA_i \| \le 1+\delta $ and therefore, assuming $\|\epsilon_i \|\le O(k/m)  C^2\le .5$, we have that $\|\bar{h}_i\|\le 2+2\delta $ and $\|h_i\|\le \|h_i\| + \|\epsilon_i \|\le 2.5+2\delta $, and $\|\tilA_i  - \trA_i \|\le 2+\delta $.  Hence, 
$$\langle h_i, \tilA_i  - \trA_i\rangle  \ge \langle \bar{h}_i, \tilA_i  - \trA_i\rangle  - (2+\delta )\|\epsilon_i \| \mbox{ and } \|\bar{h}_i\|^2 \ge (\|h_i\| -\|\epsilon_i \|)^2 \ge \|h_i\|^2  - (5+4\delta )\|\epsilon_i \|$$
This completes the proof of the lemma.
\end{proof}
\fi



%
%Then we can invoke Theorem~\ref{thm:tiger-convergence} and obtain a first-cut result regarding the convergence of OF update rule.
%
%\begin{theorem}\label{thm:making-progress}
%
%Assuming hypotheses a and b hold for $\tilA^s$, by setting $\eta < (1-\delta_0 )/\left(\max_i p_i q_i\right) = O(m/k)$ (recall $q_i = \Pr[x_i\ne 0]\approx k/m$ and $p_i = \E[x_i\sgn(x_i)|x_i\ne 0] = \Theta(1)$), we have that for any column $i$
%$$\|\tilA_i^{s+1} - \trA_i\|^2 \le (1-\gamma_i)\|\tilA_i^s - \trA_i\|^2+ O(k/n)$$
%
%where $\gamma_i= 2\eta p_i q_i \alpha \ge \Omega(\eta k/m)$. 
%%Let $\epsilon_i= 4\max_{1\le s\le N} \|\epsilon_i^s\| \le O(O(k/m)  \max_{1\le s\le N}\|\tilA^s\|^2)$, then 
%
%
%And assuming hypotheses a and b hold for all $s\ge 1$, we have that 
%
%$$\|\tilA_i^s - \trA_i\|^2 \le (1-\gamma_i)^s \cdot \|\tilA_i^0 - \trA_i\|^2+ O(k/n), \quad \forall s = 1,\dots, $$
%\end{theorem}
%%
%% Note that here we are still assuming $\|\epsilon_i^s\|$ is small for every $s$. The hope is that $\|\tilA^s\|$ should be similar to $\|\tilA\|$ and therefore $\epsilon_i$ can be bounded roughly by $O(k/m)  \|\tilA\|^2= \frac{k}{n}$, which is quite small. The rest of this section deals with this systemic error $\|\epsilon_i^s\|$ in two ways. Section~\ref{} shows how to reduce the spectral norm of $\|\tilA_i^s\|$ when it goes high, so that we could bound $\|\epsilon_i^s\|^2$. Section~\ref{} takes another approach. We try to kill entirely the systemic error term $\epsilon_i^s$ by modifying the OF update rule a bit. 








%
%\begin{algorithm}
%\caption{{\sc OF Update Rule (With Optional Whitening)}}\label{alg:main}
%\begin{algorithmic}[1]
%\REQUIRE Matrix $\tilA^0$ with  $\max_{1\le i\le m}\|\tilA_i^0 - \trA_i\|\lesssim 1/\log n$ %$\max_{i} \|\tilA_i - \trA_i\|\lesssim 1/\log n$ 
%%\ENSURE Matrix $\tilA^N$ with $\|\tilA^N- A\|_F \le \epsilon/2$ and $\max_{1\le i\le m}\|\tilA_i - \trA_i\|\lesssim 1/\log n$
%\FOR{ $s = 0$ to $N-1$}
%	\STATE $\tilA^{s+1}= $OF-update$(\tilA^s)$
%	\STATE (Optional) 
%\ENDFOR
%\end{algorithmic}
%\end{algorithm}



\subsection{Maintaining Nearness}\label{sec:nearness}





\begin{lemma}\label{lem:nowhiten}
Suppose that $\tilA^s$ is $(2\delta,2)$-\near to $\trA$. Then $\|\tilA^{s+1} - \trA\|\le 2\|\trA\|$ in Algorithm~\ref{eqn:simplestupdate}.
\end{lemma}

\begin{proof}
%First by Corollary~\ref{cor:one-step}, we have that 
%$$\|\tilA^{s+1}_i-\trA_i\| \le (1-\alpha\eta)\|\tilA^{s+1}_i-\trA_i\|  + O(k/n)\le 2(1-\alpha\eta)\delta + O(k/n) \le 2\delta$$
%First by Theorem~\ref{thm:making-progress} we know the new $\tilA^{s+1}$ is at least $(1-\gamma)^{(s+1)/2}\delta^0+O(\sqrt{k/n}) \le 2\delta_0$ close to $A$, so we only need 
%Therefore it suffices to prove that $\|\tilA^{s+1} - \trA\|\le 2\|\trA\|$.
As in the proof of the previous lemma, we will make crucial use of Lemma~\ref{lem:OF-simplified-update}. Substituting and rearranging terms we have:
\begin{eqnarray*}
\tilA^{s+1}_i - \trA_i &=&  \tilA_i^s - \trA_i - \eta g_i^s \\
& = & (1-\eta p_iq_i) (\tilA_i^s - \trA_i) + \eta p_iq_i (1-\lambda_i^s)\tilA_i^s - \eta p_i \Big( \tilA^s_{-i} \mbox{diag}(q_{i,j}) \left(\tilA_{-i}^s\right)^T \Big)\trA_i \pm \gamma
\end{eqnarray*}

Our first goal is to write this equation in a more convenient form. In particular let $U$ and $V$ be matrices such that $U_i = p_iq_i (1-\lambda_i^s)\tilA_i^s$ and $V_i = p_i \Big( \tilA^s_{-i} \mbox{diag}(q_{i,j}) \left(\tilA_{-i}^s\right)^T \Big)\trA_i$. Then we can re-write the above equation as:
$$
\tilA^{s+1}-\trA =  (\tilA^s - \trA)\mbox{diag}(1-\eta p_iq_i)+ \eta U - \eta V \pm \gamma
$$
where $\mbox{diag}(1-\eta p_iq_i)$ is the $m\times m$ diagonal matrix whose entries along the diagonal are $1-\eta p_iq_i$. 

We will bound the spectral norm of $\tilA^{s+1}-\tilA$ by bounding the spectral norm of each of the matrices of right hand side. The first two terms are straightforward to bound: $$\|(\tilA^s - \trA)\mbox{diag}(1-\eta p_iq_i)\| \le
\|\tilA^s - \trA\|\cdot (1-\eta \min_i p_iq_i) \le  2(1-\Omega(\eta k/m))\|\trA\| $$
where the last inequality uses the assumption that $p_i = \Theta(1)$ and $q_i \le O(k/m)$, and the assumption that $\|\tilA^s - \trA\|\le 2\|\trA\|$.

From the definition of $U$ it follows that $U = \tilA^s \mbox{diag}(p_iq_i(1-\lambda_i^s))$, and therefore 
$$\|U\| \le \delta \max_i p_iq_i \|\tilA^s\| = o(k/m)\cdot \|\trA\|$$
where we have used the fact that $\lambda_i^s \ge 1-\delta$ and $\delta = o(1)$, and $\|\tilA^s\| \le \|\tilA^s-\trA\|+\|\trA\| = O(\|\trA\|)$.

What remains is to bound the third term, and let us first introduce an auxiliary matrix $Q$ which we define as follows: $Q_{ii} = 0$ and $Q_{i,j} = q_{i,j}\inner{\tilA^s_i, \trA_i}$ for $i \neq j$. It is easy to verify that the following claim:
\begin{claim}
The $i$th column of $\tilA^sQ$ is equal to $\Big( \tilA^s_{-i} \mbox{diag}(q_{i,j}) \left(\tilA_{-i}^s\right)^T \Big)\trA_i$
\end{claim} 
Therefore we can write $V = \tilA^s Q\mbox{diag}(p_i)$. We will bound the spectral norm of $Q$ by bounding its Frobenus norm instead. Then from the definition of $A$, we have that:
 $$\|Q\|_F \le \left(\max_{i\neq j}q_{ij} \right) \sum_{i\neq j} \sqrt{\inner{\tilA^s_i,\trA_j}^2} = O(k^2/m^2)\|{\trA}^T\tilA^s\|_F$$
Moreover since ${\trA}^T\tilA^s$ is an $m\times m$ matrix, its Frobenius norm can be at most a $\sqrt{m}$ factor larger than its spectral norm. Hence we have
\begin{eqnarray*}
\|V\| \le \left(\max_i p_i\right)\|\tilA^s\| \|Q\| &\le& O(k^2\sqrt{m}/m^2)\|\tilA^s\|^2\|\trA\| \\
&\le & o(k/m)\|\trA\|
\end{eqnarray*}
where the last inequality uses the fact that $k = O(\sqrt{n}/\log n)$ and $\|\tilA^s\|\le O(\|\trA\|)$.  

%For the term $M_2$, its $i$-th column is equal to $\eta p_i \left(B_{-i}\mbox{diag}(q_{i,j})B^T_{-i}\right)A_i$. Let $Q\in \Re^{m\times m}$ be a matrix where $Q_{i,i} = 0$, and $Q_{i,j} = q_{i,j} \inner{B_j,A_i}$, then the term $M_2$ is
%$$
%M_2 = \mbox{diag}(\eta p_i) B Q.
%%$$
%To bound the spectral norm of $Q$, we use the fact that $q_{i,j}$'s are all small, and the Frobenius norm of $B^TA$ is at most $\sqrt{n}$ times its spectral norm (it is a matrix of rank at most $n$). Therefore:
%$$\|Q\|\le \|Q\|_F \le \max_{i\ne j} q_{i,j} \|B^TA\|_F \le \max_{i\ne j} q_{i,j} \sqrt{n} \|B^TA\| \le \max_{i\ne j} q_{i,j}6\|\tilA\|^2 = O(k^2\sqrt{n}/m^2)\|\tilA\|^2.$$
%Now the spectral norm of $M_2$ can be bounded by $\max_i\eta p_i \|B\|\|Q\| \le O(\eta k^2\sqrt{n}/m^2)\|\tilA\|^3 \le O(\eta k^2/m\sqrt{n})\|\tilA\| \le o(\eta k/m)\|\tilA\|$, where the steps are using the spectral norm bound on $A$ and the assumption that $k \le O(n/\log n)$.
%
%The term $M_3$ is negligible. Therefore we can bound the spectral norm of $\tilA^{s+1} - \trA$ as
Therefore, putting the pieces together we have: 
\begin{eqnarray*}
\|\tilA^{s+1} - \trA\| &\le & \|(\tilA^s - \trA)\mbox{diag}(1-\eta p_iq_i)\|+ \|\eta U\|+ \|\eta V\| \pm n^{-C} \\
&\le &  2(1-\Omega(\eta k/m))\|\tilA\|+ o(\eta k/m)\|\trA\| + o(\eta k/m)\|\trA\| \pm n^{-C}\\
&\le & 2\|\trA\|
\end{eqnarray*}
and this completes the proof of the lemma.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:simplestupdate-infinitesample}}
We prove by induction on $s$. Our induction hypothesis is that the theorem is true at each step $s$ and $A^s$ is $(2\delta,2)$-near to $\trA$. The hypothesis is trivially true for $s = 0$. Now assuming the inductive hypothesis is true. Recall that Corollary~\ref{cor:one-step} of Section~\ref{sec:progress} says that if $\tilA^s$ is $(2\delta,2)$-\near to $\trA$, which is guaranteed by the inductive hypothesis, by then $g_i^s$ is indeed $(\Omega(k/m), \Omega(m/k), O(k^3/mn^2))$-correlated with $\trA_i$. Invoking our framework of analysis (Theorem~\ref{thm:tiger-convergence}),  we have that 

$$\|\tilA_i^{s+1} - \trA_i\|^2\le (1-\tau) \|\tilA^{s}_i - \trA_i\|^2 + O(k^2/n^2) \le (1-\tau)^{s+1}\|\tilA^0_i - \trA_i\|^2 + O(k^2/n^2) $$

Therefore it also follows that $\tilA^{s+1}$ is $2\delta$-close to $\trA$. Then we invoke Lemma~\ref{lem:nowhiten} to prove $\tilA^{s+1}$ has not too large spectral norm $\|\tilA^{s+1}-\trA\| \le 2\|\trA\|$, which completes the induction. 
%In Section~\ref{sec:hypothesis} we complete the proof of our main theorem by proving various auxiliary lemmas we need in order to fit into the framework we developed in the previous section. In particular, 
%, we proved that if . Finally we prove that if $\tilA^s$ is $(2\delta,2)$-\near to $\trA$ then $\|\tilA^{s+1} - \trA\|\le 2\|\trA\|$ (Lemma~\ref{lem:nowhiten}). This yields our main theorem. 
%$\|\tilA_i - \trA_i\| \le \delta$, $p = \Omega(m\log m)$, new samples $y^{(1)}, y^{(2)}, ..., y^{(p)}$
%\ENSURE Matrix $H$, $\|H_i - \trA_i\| \le \delta/2$
%\STATE Let $B = ${\sc Whiten}$(\tilA, O(\sqrt{m/n}))$.
%\FOR{$i = 1$ TO $m$}
%\STATE Let $B^{(i)}$ be a matrix whose columns $B^{(i)}_j = \Proj_{\tilA_i^\perp} B_j = (I-\tilA_i\tilA_i^T)B_j$
%\STATE Initialize $Q_i\in \R^{n\times n}$ to be the all zeros matrix
%\FOR{$j = 1$ TO $p$}
%\STATE Let $S$ be the support of $y^{(j)}$
%\IF{$i \in S$}
%\STATE Let $M_S$ be the projection onto the column span of $B^{(i)}_{S\backslash\{i\}}$
%\STATE Let $r^{(j)} = (I-M_S)y^{(j)}$ be the projection of $y^{(j)}$ onto the orthogonal space of $M_S$.
%\STATE {\bf if} $\delta < 1/100k$ and $\|r^{(j)}\|> k\delta$ {\bf then} $r^{(j)} = \vec{0}$.
%\STATE Let $Q_i = Q_i + r^{(j)}(r^{(j)})^T$.%(I-M_S)y^{(j)}(y^{(j)})^T(I-M_S)$.
%\ENDIF
%\ENDFOR
%\STATE Let $H_i$ be the top singular vector of $Q_i$
%\ENDFOR
%\RETURN $H$


